CLOTHO: Directed Test Generation for Weakly Consistent Database Systems

Relational database applications are notoriously difficult to test and debug. Concurrent execution of database transactions may violate complex structural invariants that constraint how changes to the contents of one (shared) table affect the contents of another. Simplifying the underlying concurrency model is one way to ameliorate the difficulty of understanding how concurrent accesses and updates can affect database state with respect to these sophisticated properties. Enforcing serializable execution of all transactions achieves this simplification, but it comes at a significant price in performance, especially at scale, where database state is often replicated to improve latency and availability. To address these challenges, this paper presents a novel testing framework for detecting serializability violations in (SQL) database-backed Java applications executing on weakly-consistent storage systems. We manifest our approach in a tool named CLOTHO, that combines a static analyzer and a model checker to generate abstract executions, discover serializability violations in these executions, and translate them back into concrete test inputs suitable for deployment in a test environment. To the best of our knowledge, CLOTHO is the first automated test generation facility for identifying serializability anomalies of Java applications intended to operate in geo-replicated distributed environments. An experimental evaluation on a set of industry-standard benchmarks demonstrates the utility of our approach.

==> figures/abstract_anomaly2_app.tex <==
\begin{figure}[h]
%\begin{mdframed}
  \begin{subfigure}[c]{.25\textwidth}
    \centering
    \includegraphics[scale=0.255]{figures/files/internal1.pdf}
  \end{subfigure}
  %
  ~\;\;\;\;\;
  %
  \begin{subfigure}[c]{.16\textwidth}
  %$\scriptstyle H = S_0 \rightarrow 
  %S_1 \rightarrow  S_2 \rightarrow  S_3 \rightarrow  S_4 $ \\
    $\scriptstyle \bar{S}_0= \{\wrr{(\mathsf{x},f,0)},$ \\[-1mm]
  $\hspace*{5.2mm} \scriptstyle \wrr{(\mathsf{y},f,0)}\}$ 
  \\
  $\scriptstyle \bar{S}_1=\bar{S}_0\cup \{\rddp{(\mathsf{x},f,0)}\}$ \\
  $\scriptstyle \bar{S}_2=\bar{S}_1\cup \{\rddp{(\mathsf{x},f,0)}\}$\\
  $\scriptstyle \bar{S}_3=\bar{S}_2\cup \{\wrr{(\mathsf{x},f,1)}\}$\\
  $\scriptstyle \bar{S}_4=\bar{S}_3\cup \{\wrr{(\mathsf{x},f,2)}\}$
  \end{subfigure}
  %
  ~\;\;\;\; \vline\vline \;\;\;\;\;
  %
  \begin{subfigure}[c]{.25\textwidth}
    \centering
    \includegraphics[scale=0.24]{figures/files/internal2.pdf}
  \end{subfigure}
  %
  ~\;\;\;\;
  %
  \begin{subfigure}[c]{.15\textwidth}
  %$\scriptstyle H' = S'_0 \rightarrow 
  %S'_1 \rightarrow  S'_2 \rightarrow  S'_3 \rightarrow  S'_4 $ \\
    $\scriptstyle \bar{S}_0'= \{\wrr{(\mathsf{x},f,0)},$\\[-1mm]
  $\hspace*{5.2mm}\scriptstyle \wrr{(\mathsf{y},f,0)}\}$ \\
  $\scriptstyle \bar{S}_1'=\bar{S}_0'\cup \{\rdd{(\mathsf{x},f,0)}\}$ \\
  $\scriptstyle \bar{S}_2'=\bar{S}_1'\cup \{\rdd{(\mathsf{x},f,0)}\}$\\
  $\scriptstyle \bar{S}_3'=\bar{S}_2'\cup \{\wrr{(\mathsf{x},f,1)}\}$\\
  $\scriptstyle \bar{S}_4'=\bar{S}_3'\cup \{\wrr{(\mathsf{x},f,2)}\}$
  \end{subfigure}

  \caption{External (left) and internal (right)  lost update anomalies.}
    \label{fig:abstract_anomaly2_app}
  \end{figure}


==> figures/abstract_anomaly3.tex <==
\begin{figure}[h]
%\begin{mdframed}
  \begin{subfigure}{.49\textwidth}
    \centering
\includegraphics[scale=0.28]{figures/files/abstract_anomaly_3.pdf}
\caption{External Lost Update}
\label{fig:abstract_anomaly_3}
  \end{subfigure}
  %
  %
  \begin{subfigure}{.49\textwidth}
    \centering
\includegraphics[scale=0.28]{figures/files/abstract_anomaly_4.pdf}
\caption{Internal Lost Update}
\label{fig:abstract_anomaly_4}
  \end{subfigure}
%\end{mdframed}
\caption{internal and external anomalies}
\label{fig:abstract_anomaly3}
\end{figure}


==> figures/anomaly_app.tex <==
\begin{figure}[t]
  \includegraphics[width=0.29\textwidth]{figures/files/anomaly_leg.pdf}
  \qquad
  \includegraphics[width=0.65\textwidth]{figures/files/anomaly_app.pdf}
  \caption{High-level schema of anomalies constructed by \tool}
  \label{fig:anomaly_app}
\end{figure}




==> figures/ar_example.tex <==
%%-----------------
% settings
\definecolor{pgrey}{rgb}{0.26,0.25,0.28}
\definecolor{background}{rgb}{1,1,1 }
\definecolor{javared}{rgb}{0.6,0,0} % for strings
\definecolor{javagreen}{rgb}{0.2,0.45,0.3} % comments
\definecolor{javapurple}{rgb}{0.5,0,0.35} % keywords
\definecolor{javadocblue}{rgb}{0.25,0.35,0.75} % javadoc

\lstset{language=Java,
  basicstyle=\ttfamily\scriptsize,
  breaklines=true,
  backgroundcolor=\color{background},
  frame=none,
  rulecolor=\color{pgrey},
  keywordstyle=\color{javapurple}\bfseries,
  xleftmargin=-1em,
  framexleftmargin=0em,
  numberstyle=\tiny\color{pgrey},
  stepnumber=1,
  numbersep=5pt,
  stringstyle=\color{javared},
  commentstyle=\color{javagreen},
  morecomment=[s][\color{javadocblue}]{/**}{*/},
  numbers=none,
  %numberstyle=\tiny\color{pgrey},
  %stepnumber=2,
  %numbersep=6pt,
  captionpos=none,
  tabsize=1,
  showspaces=false,
  showstringspaces=false,
}


%%-----------------
% code figure

\begin {wrapfigure}{r}{0.46\textwidth}
 \begin{minipage}{.46\textwidth} 
   \begin{mdframed}[
  backgroundcolor=Main-Theme-Lightest,
     ]
  
\definecolor{background}{rgb}{0.92,0.92,0.92 }
\begin{lstlisting}[escapeinside={(*}{*)},
  backgroundcolor=\color{Main-Theme-Lightest},
]
(*$
\stx{\mathtt{payment\_txn({{id}})}\{}$*)
  (*$ 
  \sql{select}
  \fld{c\_pay\_cnt}\; 
  \sql{AS}\;
  \stx{x}\;\;
  \sql{where}
  \fld{c\_id={id}};$*)
  (*$
  \mathtt{if(size(x)>0)\{}
  $*)
    (*$
  \sql{update} 
  \sql{set}
  $
  $\stx{\fld{c\_pay\_cnt}=\pi(\fld{c\_pay\_cnt},\sigma(x,1))+1}
  $*)
    (*$
  \sql{where}
    \fld{c\_id={id}\}\}}
$*)
\end{lstlisting}
\vspace{-2mm}
\end{mdframed}
\end{minipage}
\vspace{-2mm}
\caption{Payment txn compiled to \ir}
\label{fig:ar_example}
\end{wrapfigure}


==> figures/ar_syntax_app.tex <==
\begin {figure}[h]
 \begin{minipage}{.9\textwidth} 
   \begin{mdframed}[
  backgroundcolor=Main-Theme-Lightest,
     ]
  \begin{mathpar}
  \footnotesize
  \begin{array}{lcl}
  \multicolumn{3}{c}{
    \stx{p} \in \mathtt{Parameters} \qquad
    \stx{x} \in \mathtt{RowListVars} \qquad
    \stx{f} \in \mathtt{Fields} \qquad 
    %\stx{l} \in \stx{Loop IDs} \quad 
    \stx{A} \in \{\tt{min, max, count}\} } \\
  \multicolumn{3}{c}{
    \stx{T} \in \mathtt{Tname} \qquad 
    \oplus \in \{+, -, \times, /\} \qquad 
    \odot \in \{<, \leq, =, >, \geq\} \qquad 
    \circ \in \{\wedge, \vee\} }\\
\\
%
\phi & \coloneqq & \stx{v\odot v} 
\ALT 
\neg\phi \ALT \phi\circ\phi 
\ALT \mathtt{true} \ALT \mathtt{false}
\\
\stx{v} & \coloneqq & 
\stx{v\oplus v}
\ALT \intt 
\ALT \stx{p} 
\ALT \stx{\mathtt{\pi}(f,{r})}  
\ALT \stx{\mathtt{abs}^{\phi}}
\ALT \stx{\mathtt{size}(x)}
\ALT \stx{\mathtt{iter}}
\ALT \stx{f}
\\
\stx{r} & \coloneqq & 
\stx{\sigma(x,\natt)} 
\\
\stx{q} & \coloneqq & \sql{select} \stx{f}\; \sql{as} \stx{x}\;
\sql{where} \stx{\phi} 
\ALT
\sql{select} \stx{A(f)}\; \sql{as} \stx{x}\;
\sql{where} \stx{\phi} 
\ALT 
\\
        & & \sql{update} \sql{set}
        \stx{f=v} \; \sql{where} \stx{\phi}
\ALT
\sql{insert} \sql{values} \stx{\overline{f}=\overline{v}} 
\ALT
 \sql{delete} \sql{where} \stx{\phi}
\\
\stx{c} & \coloneqq & 
\stx{q}
\ALT
\mathtt{if(\phi)}\{c\}
\ALT
\mathtt{iterate}(\natt)\{c\} 
\ALT
c;c
\\
\stx{txn} & \coloneqq & \stx{T(\overline{p})\{c\}}

\end{array}
  \end{mathpar}
\end{mdframed}
\end{minipage}
\caption{Syntax of transactional programs written in the abstract
\label{fig:syntax_app}
representaiton (\ir)}
\end{figure}


==> figures/arbit_ser.tex <==
\begin{wrapfigure}[9]{r}{0.33\textwidth}
  \vspace{-5mm}
  \begin{mdframed}[backgroundcolor=Main-Theme-Lightest]
  \centering
\includegraphics[width=1\textwidth]{figures/files/arbit_ser.pdf}
\end{mdframed}
  \vspace{-3mm}
  \caption{A non-serial (left) and a serial (right) execution}
\label{fig:arbit_ser}
\end{wrapfigure}


==> figures/complete_issue.tex <==
\begin{figure}[t]
  \begin{subfigure}{0.45\textwidth}
  \includegraphics[scale=0.26]{figures/files/complete.pdf}
\end{subfigure}
~  
~
\begin{subfigure}{0.45\textwidth}
  \includegraphics[scale=0.26]{figures/files/complete2.pdf}
  \end{subfigure}
  \caption{the complete issule}
    \label{fig:complete_issue}
  \end{figure}


==> figures/cycles_app.tex <==
\begin{figure}[h]
%\begin{mdframed}
  \begin{subfigure}[c]{.25\textwidth}
    \centering
    \includegraphics[scale=0.26]{figures/files/cycle1.pdf}
  \end{subfigure}
  %
  ~
  %
  \begin{subfigure}[c]{.25\textwidth}
    \centering
    \includegraphics[scale=0.26]{figures/files/cycle2.pdf}
  \end{subfigure}
  %
  ~
  %
  \begin{subfigure}[c]{.25\textwidth}
    \centering
    \includegraphics[scale=0.26]{figures/files/cycle3.pdf}
  \end{subfigure}
  \caption{Examples of valid (left, middle) and invalid (right) cycles where
  $\folD\in\{\folwr,\folrw,\folww\}$}
    \label{fig:cycles_app}
  \end{figure}


==> figures/denote_b.tex <==
 \begin{figure}[h]
   \caption{FOL encoding of a given conditional $\phi$, specialized to transaction instance t}
    \label{fig:denote_b}
\end{figure}




==> figures/denote_v.tex <==
%
% FIGURE DENOTE^V
%
%
\begin{figure}[h]
 \begin{minipage}[b]{.49\textwidth}
\begin{mdframed}[backgroundcolor=Main-Theme-Complement]
  \centering
        \begin{mathpar}
        \small
        \begin{array}{lcl}
          \V{p}{} & = & (\mathsf{true},\fol{\eta}(t,p)) \\
          \V{f}{} & = & (\mathsf{true},\fol{\rho}(r,f,r_v(f))) \\
          \V{n}{} & = & (\mathsf{true},\stx{n}) \\
          \V{\mathsf{abs}^{\phi}}{} & = &
          (\mathsf{true},\stx{\fol{\alpha}(t,\mathsf{abs}^{\phi})}) \\
          \V{\mathsf{iter}}{} & = & (\mathsf{true},\fol{\beta}(c,\mathsf{iter})) \\
          \V{\pi(f,\sigma(x,n))}{} & = 
                                               &
                                               (\exists{\mathring{\stx{r}}},\mathring{\stx{r_v}}.\;
                                               \fol{\nu}(t,{\mathring{\stx{r}}},{\mathring{\stx{r_v}}},n), 
                                            \\ & &
                                               \fol{\rho}_{\mathring{\stx{r}}}(f,{\mathring{\stx{r_v}}}(f))
\\
          \V{v_1\oplus v_2}{} & = & let \quad \V{v_1}{} = (\foldcond_1,\foldval_1) \\ & &
          \,\,\,\,\,\; \quad \V{v_2}{} = (\foldcond_2,\foldval_2) \\ 
& &in \quad (\foldcond_1\wedge\foldcond_2,(\foldval_1\oplus\foldval_2))

	\end{array}
        \end{mathpar}
\end{mdframed}
\end{minipage}
\quad
  \begin{minipage}[b]{.45\textwidth}
  \begin{mdframed}[backgroundcolor=Main-Theme-Complement]
    \centering
        \begin{mathpar}
        \small
        \begin{array}{lcl}
          \B{\stx{\mathsf{true}}}{} & = & \mathsf{true} \\
          \B{\mathsf{false}}{} & = & \mathsf{false} \\
          \B{\stx{\phi_1 \circ \phi_2}}{} & = & \B{\phi_1}{} \circ
\B{\phi_2}{} \\
          \B{\stx{\neg{\phi}}}{} & = & \neg{\B{\stx{\phi}}{}} \\
          \B{\stx{v_1 \odot v_2}}{} & = &
          let \quad \V{v_1}{} = (\foldcond_1,\foldval_1) \\ & &
          \,\,\,\,\;\, \quad \V{v_2}{} = (\foldcond_2,\foldval_2) \quad \\ & &
          in \;\;\;\;\;
          \foldcond_1\wedge\foldcond_2
          \wedge (\foldval_1\odot\foldval_2)
        \end{array}
        \end{mathpar}
\end{mdframed}
  \end{minipage}
    \caption{
      Definition of functions
      $\B{}{t,c,r,r_v}$ and 
      $\V{}{t,c,r,r_v}$. 
    Subscripts are omitted for perspicuity.}
    \label{fig:denote_v}
\end{figure}
%




==> figures/fol_eval.tex <==
%
% FIGURE DENOTE^B
%
\begin{figure}[t]
  \begin{minipage}[b]{.39\textwidth}
    \begin{mdframed}[
    backgroundcolor=Main-Theme-Complement,
    innerleftmargin=0cm,
    innerrightmargin=0cm,
    innertopmargin=0pt]
    \vspace{0.3mm}
    \centering
        \begin{mathpar}
        \footnotesize
        \begin{array}{lcl}
          \B{\stx{true}}{t,r} & = & \sql{true} \\
          \B{\stx{false}}{t,r} & = & \sql{false} \\
          \B{\stx{\phi_1 \circ \phi_2}}{t,r} & = & \B{\phi_1}{t,r} \circ
\B{\phi_2}{t,r} \\
          \B{\stx{\neg{\phi}}}{t,r} & = & \neg{\B{\stx{\phi}}{t,r}} \\
          \B{\stx{v_1 \odot v_2}}{t,r} & = &
          let \quad \V{v_1}{t,r} = (\foldcond_1,\foldval_1) \\ & &
          \,\,\,\,\;\;\, \quad \V{v_2}{t,r} = (\foldcond_2,\foldval_2) \\ & &
          in \\ & &

          \foldcond_1\wedge\foldcond_2
          \wedge (\foldval_1\odot\foldval_2)
           \\
        \end{array}
        \end{mathpar}
\end{mdframed}
  \end{minipage}
%    \caption{FOL encoding of a given conditional $\phi$, specialized to transaction instance t}
%    \label{fig:denote_b}
%
%
% FIGURE DENOTE^V
%
%
  \begin{minipage}[b]{.54\textwidth}
\begin{mdframed}[
  backgroundcolor=Main-Theme-Complement,
    innerleftmargin=0cm,
    innerrightmargin=0cm,
    innertopmargin=0pt]
  \centering
        \begin{mathpar}
        \footnotesize
        \begin{array}{lcl}
          \V{p}{t} & = & (\sql{true},\folparam{p}(\stx{t})) \\
          \V{f}{t,r} & = & (\sql{true},\folproj{f}(\stx{r})) \\
          \V{n}{t} & = & (\sql{true},\stx{n}) \\
          \V{\stx{abs}^{\phi^i}}{t} & = & (\B{\phi[\mathring{\folabs}/i]}{t},\mathring{\folabs}) \\
          \V{proj_f(next^n(v_{\hat{r}}))}{t} & = 
                                               & (\exists{\mathring{\stx{r}}}.\;
                                               \varproj_{\stx{v_{\hat{r}}}}\stx{(n,\mathring{r},t)}
\wedge \\ & &
\forall_{\stx{n'<n,r'}}.\varproj_{\stx{v_{\hat{r}}}}\stx{(n',r',t)}
\Rightarrow 
 \stx{r'}\neq\mathring{\stx{r}},
 \\ & &
\folproj{f}(\mathring{\stx{r}})) \\
          
	  \V{proj_f(loop^l(v_{\hat{r}}))}{t} & =
                                         & \stx{(\exists{\mathring{r},\mathring{n}}.\;
\varproj_{\stx{v_{\hat{r}}}}(\mathring{n},\mathring{r},t),
\folproj{f}(\mathring{r}))} \\
%
%
%          \V{(\phi,v_1,v_2)}{t,r} & = & if\;\; \B{\phi}{t,r} \;\; then \;\;
%\V{v_1}{t,r}
%\\ 
%& & \qquad\qquad\;\,\, else\;\,\,\, \V{v_2}{t,r}
%\\
%          \V{v_1\oplus v_2}{t,r} & = & let \quad \V{v_1}{t,r} = (\foldcond_1,\foldval_1) \\ & &
%          \,\,\,\,\;\,\; \quad \V{v_2}{t,r} = (\foldcond_2,\foldval_2) \quad in \\ 
%& &(\foldcond_1\wedge\foldcond_2,(\foldval_1\oplus\foldval_2))
%
	\end{array}
        \end{mathpar}
\end{mdframed}
\end{minipage}
\caption{Formal definition of evalation function $\B{}{t,r}$ (left)  
and extraction function $\V{}{t,r}$ (right)}
    \label{fig:fol_eval}
\end{figure}
%
%
%
%
%
%
%


==> figures/fol_rule_example.tex <==
\begin{wrapfigure}[10]{r}{0.46\textwidth}
  \begin{mdframed}[backgroundcolor=Main-Theme-Complement]
  \begin{minipage}{0.5 \textwidth}
  \centering
  %%
%\rulelabel{rw-select-update}
$$
\FOLRULE{
  \stx{c_1 \equiv (\sql{select}(f)\; \sql{as}
  x\;\sql{where} \phi_1^w, \folpath{1}) } \\
  \stx{c_2 \equiv (\sql{update}\sql{set}
  (f=n)\;\sql{where} \phi_2^w, \folpath{2}) } \\
  \stx{
    \folparent(c_1)=t_1 \qquad \folparent(c_2)=t_2 }
    \\
    \stx{t_1 \neq t_2}
  \qquad
}
%% ------------------------------------------------------------------------------------------------
  {
    \eta^{\folrw\rightarrow}_{c_1,c_2} =
    \folrw(c_1,c_2) \Rightarrow
  }
  {
    \qquad
    \stx{
      \B{\folpath{1}}{t_1}
      \wedge \B{\folpath{2}}{t_2}
    }
  \stx{
    \wedge
    \exists r.
    \B{\phi_1^w}{t_1,r}
    \wedge \B{\phi_2^w}{t_2,r}
  % \wedge (\bigwedge \folproj{f(i)}(r)=\foldval^i_2)
  }
  }
$$

  \end{minipage}
\end{mdframed}
%\fcolorbox{black}{Main-Theme-Lighter}{\textrm{\sc{\color{black} #1}}}
  \caption{{{\textrm{\sc{\color{black}
  rw-select-update}}}} }
    \label{fig:fol_rule_example}
  \end{wrapfigure}


==> figures/full_operational_semantics_B.tex <==
\begin{figure}[h]
  \begin{minipage}{.38\textwidth}
  \begin{mdframed}[backgroundcolor=Main-Theme-Lightest]
    \centering
        \begin{mathpar}
        \small
        \begin{array}{lcl}
          \B{\mathsf{true}}{}& = & \mathsf{true}\\[1mm]
          \B{\mathsf{false}}{}& = & \mathsf{false}\\[1mm]
          \B{\phi_1 \circ \phi_2}{}& = & \B{\phi_1}{} \circ
          \B{\phi_2}{}\\[1mm]
          \B{\neg\phi}{}& = &\neg\B{\phi}{} \\[1mm]
          \B{v_1\odot v_2}{} & = & 
          \I{v_1}{} \odot \I{v_2}{}
          %\exists n_1,n_2. \;\;
          %n_1\in\I{v_1}{\Theta}  \wedge
          %n_2\in\I{v_2}{\Theta} 
          %\wedge (n_1\odot n_2)
        \end{array}
        \end{mathpar}
  \end{mdframed}
  \end{minipage}
    \caption{Boolean evaluation $\B{}{\theta,\delta,r_k}$ used in our 
    operational semantics. Subscripts are omitted for perspicuity.
}
    \label{fig:b_definition}
\end{figure}


==> figures/full_operational_semantics_I.tex <==
\begin{figure}[t]
\begin{minipage}[b][][b]{.38\textwidth}
  \begin{mdframed}[backgroundcolor=Main-Theme-Lightest]
    \centering
        \begin{mathpar}
        \small
        \begin{array}{lcl}
          \B{\mathsf{true}}{}& = & \mathsf{true}\\[1mm]
          \B{\mathsf{false}}{}& = & \mathsf{false}\\[1mm]
          \B{\phi_1 \circ \phi_2}{}& = & \B{\phi_1}{} \circ
          \B{\phi_2}{}\\[1mm]
          \B{\neg\phi}{}& = &\neg\B{\phi}{} \\[1mm]
          \B{v_1\odot v_2}{} & = & 
          \I{v_1}{} \odot \I{v_2}{}
        \end{array}
        \end{mathpar}
  \end{mdframed}
  \end{minipage}
  \quad
  \begin{minipage}[b][][b]{.53\textwidth}
  \begin{mdframed}[backgroundcolor=Main-Theme-Lightest]
    \centering
        \begin{mathpar}
        \small
        \begin{array}{lcl}
          \I{v_1\oplus v_2}{} & = &  \I{v_1}{} \oplus \I{v_2}{}\\
          \I{n}{}& = & \stx{n}  \\
           \I{p}{}& = &\eta(\stx{p}) \\
           \I{\stx{\pi(f,\sigma(x,n))}}{}& = & 
           let \;\; (\rec_k',\rec_v') = \nu(\theta(x),n) \;\; in \\ & &
           \stx{\rho(\rec_k',\rec_v')(f)} \\
           \I{\mathtt{abs}^{\phi}}{} & = & \alpha(\mathtt{abs^{\phi}})\\
           \I{\mathtt{size}(x)}{} & = & |\theta(x)|\\
           \I{\mathtt{iter}}{} & = & \beta(\mathtt{iter})\\
           \I{f}{}& = & \rho(\rec_k,\delta(\rec_k))(f)
        \end{array}
        \end{mathpar}
  \end{mdframed}
  \end{minipage}
  \caption{Boolean evaluation $\B{}{\theta,\delta,\rec_k}$ (left) and integer
    evaluation $\I{}{\theta,\delta,\rec_k}$ (right) functions, used in 
    our operational semantics. Subscripts are omitted for perspicuity.}
    \label{fig:i_definition}
\end{figure}


==> figures/inverse_fol_rule_example.tex <==
\begin{figure}[h]
\begin{minipage}[b]{0.55\textwidth}
  \begin{mdframed}[backgroundcolor=Main-Theme-Complement]
  \centering
  %%
%\rulelabel{rw-select-update}
$$
\FOLRULE{
  \stx{c_1 \equiv (\sql{select}(f)\; \sql{as}
  x\;\sql{where} \phi_1^w, \folpath{1}) } \\
  \stx{c_2 \equiv (\sql{update}\sql{set}
  (f=n)\;\sql{where} \phi_2^w, \folpath{2}) } \\
  \stx{
    \folparent(c_1)=t_1 \qquad \folparent(c_2)=t_2 }
    \qquad
    \stx{t_1 \neq t_2}
}
%% ------------------------------------------------------------------------------------------------
  {
    \eta^{\rightarrow\folwr}_{c_2,c_1} =
    \stx{
      (\B{\folpath{1}}{t_1}
      \wedge \B{\folpath{2}}{t_2}
    } 
      \stx{
    \wedge
    \exists r.
    \B{\phi_1^w}{t_1,r}
    \wedge \B{\phi_2^w}{t_2,r}
  % \wedge (\bigwedge \folproj{f(i)}(r)=\foldval^i_2)
  }
  }
  {
    \wedge \foltime(c_1)>\foltime(c_2))  
    \Rightarrow 
    \folwr(c_2,c_1)
  }
$$
\vspace{0.5mm}
\end{mdframed}
%\fcolorbox{black}{Main-Theme-Lighter}{\textrm{\sc{\color{black} #1}}}
  \caption{{{\textrm{\sc{\color{black}
  select-update-wr}}}} }
    \label{fig:inverted_fol_rule_example}
\end{minipage}
  \end{figure}


==> figures/serial_def.tex <==
\begin{figure}[t]
%\begin{mdframed}
  \begin{subfigure}[t]{.3\textwidth}
    \centering
\includegraphics[scale=0.27]{figures/files/serial_example1.pdf}
\caption{non-serial execution}
\label{fig:serial_def1}
  \end{subfigure}
  %
  ~\;\;
  %
  \begin{subfigure}[t]{.3\textwidth}
    \centering
\includegraphics[scale=0.27]{figures/files/serial_example2.pdf}
\caption{serial execution}
\label{fig:serial_def2}
  \end{subfigure}
  %
  ~\;\;
  %
  \begin{subfigure}[t]{.3\textwidth}
    \centering
\includegraphics[scale=0.27]{figures/files/serial_example3.pdf}
\caption{serializable execution}
\label{fig:serial_def3}
  \end{subfigure}
  \caption{Events generated in concurrent executions of
    $\txn{payment}$ transactions. }
    \label{fig:serial_def}
  \end{figure}


==> figures/serializability_example_app.tex <==
\begin{figure}[h]
%\begin{mdframed}
  \begin{subfigure}[b]{.25\textwidth}
    \centering
    \includegraphics[scale=0.255]{figures/files/serializable.pdf}
  \end{subfigure}
  %
  ~\;\;\;\;\;
  %
  \begin{subfigure}[b]{.15\textwidth}
  %$\scriptstyle H = S_0 \rightarrow 
  %S_1 \rightarrow  S_2 \rightarrow  S_3 \rightarrow  S_4 $ \\
    $\scriptstyle \bar{S}_0= \{\wrr{(\mathsf{x},f,0)},$ \\[-1mm]
  $\hspace*{5.2mm} \scriptstyle \wrr{(\mathsf{y},f,0)}\}$ 
  \\
  $\scriptstyle \bar{S}_1=\bar{S}_0\cup \{\rdd{(\mathsf{y},f,0)}\}$ \\
  $\scriptstyle \bar{S}_2=\bar{S}_1\cup \{\rdd{(\mathsf{x},f,0)}\}$\\
  $\scriptstyle \bar{S}_3=\bar{S}_2\cup \{\wrr{(\mathsf{y},f,1)}\}$\\
  $\scriptstyle \bar{S}_4=\bar{S}_3\cup \{\wrr{(\mathsf{x},f,1)}\}$
  \end{subfigure}
  %
  ~\;\;\;\; \vline\vline \;\;\;\;\;
  %
  \begin{subfigure}[b]{.25\textwidth}
    \centering
    \includegraphics[scale=0.255]{figures/files/serial.pdf}
  \end{subfigure}
  %
  ~\;\;\;\;\;
  %
  \begin{subfigure}[b]{.15\textwidth}
  %$\scriptstyle H' = S'_0 \rightarrow 
  %S'_1 \rightarrow  S'_2 \rightarrow  S'_3 \rightarrow  S'_4 $ \\
    $\scriptstyle \bar{S}_0'= \{\wrr{(\mathsf{x},f,0)},$\\[-1mm]
  $\hspace*{5.2mm}\scriptstyle \wrr{(\mathsf{y},f,0)}\}$ \\
  $\scriptstyle \bar{S}_1'=\bar{S}_0'\cup \{\rdd{(\mathsf{y},f,0)}\}$ \\
  $\scriptstyle \bar{S}_2'=\bar{S}_1'\cup \{\wrr{(\mathsf{y},f,1)}\}$\\
  $\scriptstyle \bar{S}_3'=\bar{S}_2'\cup \{\rdd{(\mathsf{x},f,0)}\}$\\
  $\scriptstyle \bar{S}_4'=\bar{S}_3'\cup \{\wrr{(\mathsf{x},f,1)}\}$
  \end{subfigure}

  \caption{A serializable execution (left) and its equivalent serial execution
  (right)}
    \label{fig:serializability_example_app}
  \end{figure}


==> sections/full_fol_encoding.tex <==
\newpage 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Static Anomaly Generation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We now turn to the question of how to detect dependency cycles and construct 
independent serializability anomalies in \ir\ programs. 
We adopt the approach presented in~\citet{KR18} and~\citet{BR18} 
and reduce (the bounded version of) our problem to constructing an FOL formula 
$\varphi_{\mathbb{C}}$ from a given \ir\ program.  This formula includes variables for each of the dependency,
visibility, and arbitration constraints that can appear during the
program's execution, and is designed such that the assignments to
these variables in any satisfying model for $\varphi_{\mathbb{C}}$  can be used
to reconstruct an execution of the original program.
This allows us to use an off-the-shelf SAT solver to efficiently check for anomalous
executions in the given program.
Given bounds $max_p$, $max_t$ and $max_c$,
the shape of the full formula is a conjunction of five clauses, 
each representing a different aspect of the encoding:
$$\varphi_{\mathbb{C}}\overset{\Delta}{\equiv} 
\folphi{context}
\wedge
\folphi{db} 
\wedge \folphi{$\rightarrow$dep} \wedge
\folphi{dep$\rightarrow$}
\wedge 
\bigvee_{\substack{0\leq k_p\leq max_p\\2\leq k_t\leq max_t\\3\leq k_c\leq max_c}}
\!\!\!\!\!\folphi{anomaly}^{k_p,k_t,k_c}$$


The set of constraints on variables and functions, 
corresponding valid executions of any database program is captured by $\folphi{context}$.
Clause $\folphi{DB}$ is a set of user-defined constraints on acceptable database records.
$\folphi{dep$\rightarrow$}$ 
and 
$\folphi{$\rightarrow$dep}$ 
respectively capture the necessary and sufficient conditions for establishing dependency
relations between command instances from the given program. 
Following our definition of independent serializability anomalies in
\autoref{sec:model}, using $\folphi{anomaly}^{k_p,k_t,k_c}$ we force the solver 
to instantiate a serial execution of $k_p$ transactions that leads to
concurrent execution of $k_t$ transactions within which 
a dependency cycle of length $k_c$ is formed.
A high-level overview of such an instantiation is presented in 
\autoref{fig:anomaly_app}. 

In the remaining of this section, we will lay the formal groundwork and present
each clause of $\varphi_{\mathbb{C}}$ in detail. 


\input{figures/anomaly_app}


















%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{preliminaries}
%%%%%%%%%%%%%%%%%%%%%%%%%%
We assume uninterpreted sorts for transactions
($\txnsort$), commands ($\opsort$) and records ($\rowsort$).
Finite sort $\mathbb{F}$ is also defined to capture table fields
according to the specified data model.
Similarly, based on the syntax of the input program,
for each rowList variable $x$, each abstract variable $\mathsf{abs^\phi}$,  
each transaction input parameter $p$ and each iteration variable
$\mathsf{iter}$, we associate finite sorts respectively 
denoted by  $\mathbb{X}$, $\mathbb{A}$, $\mathbb{P}$ and $\mathbb{I}$.
Finally, finite sorts  $\mathbb{T}$ and $\mathbb{C}$ are created to capture
transaction types and command types. 

We define function $\mathsf{txn():\opsort\rightarrow\txnsort}$ to relate command instances to their encapsulating
transaction instance. 
We also define appropriate typing functions, using which
each transaction instance $t\in\txnsort$ 
is associated to a transaction type (similarly for command instances $c\in\opsort$). 
    For example, transaction type  {\textcolor{orange}{$\mathsf{payment}$}}$~\in\mathbb{T}$
    is associated to all instances of payment transaction and command type 
    {\textcolor{orange}{$\mathsf{payment\_c2}$}}$~\in\mathbb{C}$
    is associated to the second command in such transactions. We assume all
    loops are unrolled up to a bound specified by users. We lastly assume a
    function $\Lambda: \opsort\rightarrow \phi$ which returns 
    the conjunction of all conditionals that must be satisfied before a command
    instances is reached by the program's control flow. 

       We define functions $\folversion{wr}:\rowsort\times\opsort\rightarrow
       r_v$ and $\folversion{rd}:\rowsort\times\opsort\rightarrow r_v$ 
        where we use $r_v:\mathbb{F}\rightarrow\natt$ to denote a
       function from field names to natural version numbers. 
       $\folversion{wr}$ and $\folversion{rd}$
       respectively capture the version of a row that a command instance 
       writes or witnesses. We use $\folversionsub{wr}{r,f}(c)$ to denote
       $\folversion{wr}(r,c)(f)$.
We also define $\fol{\rho}: \rowsort\times\mathbb{F}\times\natt\rightarrow\intt$
to relate different versions of row instances to concrete values. We use
$\fol{\rho}_{r}(f,n)$ to denote $\fol{\rho}(r,f,n)$.
We define syntactic sugars $\folalive{_{rd}}{}:\rowsort\times \opsort\rightarrow \booll$ and
$\folalive{_{wr}}{}:\rowsort\times \opsort\rightarrow \booll$  to capture the
       liveness of the read or written row in a particular command instance.
       Formally, 
       $$\folalive{_{\mathsf{op}}}{}(r,c)\Leftrightarrow\fol{\rho}_{r}(f^\dagger,
       \folversionsub{op}{r,f^\dagger}(c))=1,\qquad
       \mathsf{op}\in\{wr,rd\}$$

       In accordance with the definition of 
functions and predicates presented in \autoref{sec:model},
we now define the following FOL functions:

\begin{itemize}
  \item
      $\fol{\omega}_{}: \txnsort\times\natt\rightarrow \opsort$ to
      relate a transaction instance to the ordered list of its command
      instances.
  \item $\fol{\eta}:\txnsort\times \mathbb{P}\rightarrow\intt$ to
relate each transaction instance to concrete input arguments. 
\item 
   $\fol{\alpha}:\txnsort\times\mathbb{A}\rightarrow\intt$ 
   to concretize abstract variables called in a transaction instance. 
 \item
   $\fol{\tau}:\opsort\rightarrow\natt$ to relate a command
      instance to the partition it is executed at.
  \item $\fol{\beta}:\opsort\times\mathbb{I}\rightarrow \intt$ to relate
    iteration variables in a command instance to concrete values. 
    
 \item 
 $\fol{\nu_x}:\txnsort\times\rowsort\times
       r_v\times\natt\rightarrow \booll$
       to capture the \emph{ordered set} of rows and their witnessed versions 
       stored in variable $x\in\mathbb{X}$ in a transaction instance. 
       For example, if $\fol{\nu_x}(t,r,r_v,3)$ is true, then transaction $t$ has
       performed a $\sql{select}$operation the result of which is stored in a variable
       $x$. It also means that $r$ is the third row  in $x$ and $t$ has
       witnessed $r_v$ as the version $r$. 
  \item $\vis:\opsort\times\opsort\rightarrow\booll$ 
to capture visibility relation between command instances.
  \item 
$\ar:\opsort\times\opsort\rightarrow\booll$ 
to capture 
arbitration relation 
between command instances.
  
  \item 
      $\folwr,\folrw$ and $\folww$ all of signature
      $\rowsort\times\mathbb{F}\times\opsort\times\opsort\rightarrow\booll$ to
      capture dependencies on a specific field of a row, between two command
      instances. We may denote the first two
      arguments as superscripts, e.g.
      $\folrw^{r,f}(c_1,c_2)$ instead of $\folrw(r,f,c_1,c_2)$.

  
    \item 
      $\folst:\opsort\times\opsort\rightarrow\booll$  is defined 
      to relate commands belonging to the same transaction instance. $\folstp$ is
      similarly defined which also takes into account the data dependency
      between the related command instances. 
  
  
  
  
  \end{itemize}



We are now ready to introduce the core 
encoding function $\V{}{t,c,r,r_v}$ in \autoref{fig:denote_v} (left) which
constructs FOL formulae corresponding values in \ir, alongside the conditions
that must be satisfied for a successful construction. 
Similarly and based on the definition of $\V{}{}$, we introduce function 
$\B{}{t,c,r,r_v}$ in \autoref{fig:denote_v}
(right). 
$\B{\phi}{t,c,r,r_v}$ is satisfiable if and only if $\phi$ is valid in 
the transaction instance $t$.  

%
 \input{figures/denote_v}
%






 


%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Components of FOL Encoding}
%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section we present detailed descriptions of each clause in 
$\varphi_{\mathbb{C}}$:
$$\varphi_{\mathbb{C}}\overset{\Delta}{\equiv} 
\folphi{context}
\wedge
\folphi{db} 
\wedge \folphi{$\rightarrow$dep} \wedge
\folphi{dep$\rightarrow$}
\wedge 
\bigvee_{\substack{0\leq k_p\leq max_p\\2\leq k_t\leq max_t\\3\leq k_c\leq max_c}}
\!\!\!\!\!\folphi{anomaly}^{k_p,k_t,k_c}$$















%%
%%
\subsubsection{\normalfont $\folphi{anomaly}$}
%%
%%


We define the following proposition 
which specifies that an independent serializability anomaly exists, that
is consisted of
\color{dark-red}
$k_p$ serially executed transactions
\color{dark-blue}
and 
$k_t$ concurrent transactions that manifest a dependency cycle of
length $k_c$.
\color{dark-green}
It is required that all serializable transactions are executed before the cycle.
\color{black}

$$\folphi{anomaly}^{k_p,k_t,k_c} \overset{\Delta}{\equiv} 
\color{dark-red}
\exists t_1,...,t_{k_p}.\!\!\!\!\bigwedge_{1\leq i\leq
k_p}\!\!\!\folphi{ser}(t_i) 
\color{black}
\wedge 
\color{dark-blue}
\exists t'_{1},...,t'_{k_t}.\;
\folphi{cycle}^{k_c}(t'_1,...,t'_{k_t})
\color{black}
\wedge
\color{dark-green}
\bigwedge_{\substack{1\leq i \leq
k_p\\1\leq j\leq 
k_t}}\bigwedge_{\substack{c,c'\in\opsort\\\txnR(c)=t_i\\\txnR(c')=t'_j}}
\!\!\!\!\ar(c,c') $$




In the above formula,
$\folphi{ser}(t)$
specifies the serializability of transaction $t$ with respect to other transaction
instances. It is defined using $ \folphi{rc}(c)$, $ \folphi{rr}(c)$ and $
\folphi{lin}(c)$ which are consistency and
isolation guarantees (discussed in \autoref{sec:model}) \emph{refined for a single command $c$}: 
\begin{equation*}
  \begin{array}{rcl}
    \folphi{rc}(c) &  \overset{\Delta}{\equiv} &  
  \bigwedge_{c',c''\in\opsort}
  (\txnR(c')=\txnR(c'')\wedge
  \vis(c',c)) \Rightarrow \vis(c'',c)
\\
    \folphi{rr}(c) & \overset{\Delta}{\equiv}  &
  \bigwedge_{c',c''\in\opsort}
  (\txnR(c')=\txnR(c)\wedge
  \vis(c'',c)) \Rightarrow \vis(c'',c')
\\
    \folphi{lin}(c) & \overset{\Delta}{\equiv}  &
  \bigwedge_{c'\in\opsort} 
  \ar(c',c) \Rightarrow \vis(c',c)
\\
    \folphi{ser}(t) & \overset{\Delta}{\equiv}  &
    \bigwedge_{c\in\opsort} (\txnR(c)=t)
\Rightarrow \folphi{rc}(c)\wedge\folphi{rr}(c)\wedge\folphi{lin}(c)
\end{array}
\end{equation*}



We finally introduce $\folphi{cycle}^{k_c}(t_1,...,t_{k_t})$ which is intended 
to instantiate $k_c$ commands forming a dependency cycle within the given
transactions:
  \begin{align*}
\folphi{cycle}^{k_c}(t_1,...,t_{k_t})
 \overset{\Delta}{\equiv}\;
 &
\exists c_1,...,c_{k_c}. 
\bigwedge_{1\leq i\leq k_c}
(\txnR(c_i)\in\{t_1,...,t_{k_t}\}) \wedge 
\\[-2mm]
 & \folst(c_1,c_{k_c}) \wedge \folD(c_1,c_2)\wedge \folD(c_{k_c-1},c_{k_c}) \wedge
\!\bigwedge_{2\leq
i<{k_c-1}}\!(\folst(c_i,c_{i+1})\vee\folD(c_i,c_{i+1})) 
\end{align*}
Our definition of dependency cycles is based on \autoref{sec:model} and
enforces that $k_c$ edges circularly exists between commands, 
at least two of which are in $\{\folwr,\folrw,\folww\}$ and one is a $\folst$
edge.

\autoref{fig:abstract_anomaly} presents examples of dependency cycles detected
by \tool.
\autoref{fig:abstract_anomaly_1} depicts a scenario where the
$\sql{select}$command from
$\txn{oneRead}$ transaction witnesses the intermediate value written by
$\txn{twoWrites}$ transaction. \tool\ automatically determines the
execution order of commands (shown as circled numbers)
and input transaction parameters 
required for manifestation of the anomaly (in this case it suffices that
$\mathsf{k_1=k_2=k_3}$).
%
Anomaly depicted in 
\autoref{fig:abstract_anomaly_2} occurs when an update
from transaction $\txn{twoWrites}'$ is executed at a node which
then becomes disconnected from the network to form {\color{dark-red} replica 1}.
%
Assuming that clients can access the rest of the network on
{\color{weborange} replica 2}, the remaining commands need to be
submitted to available nodes in the specified order in order to
trigger the depicted serializability anomaly. 
This anomaly does not occur when network partitioning is not possible. 

\tool\ users may opt out from reports of external serializability anomalies in their
programs, in which case, $\folst$ is replaced with $\folstp$ in
$\folphi{cycle}$.
\autoref{fig:abstract_anomaly_3} and \autoref{fig:abstract_anomaly_4}
respectively present the
cycles detected for external and internal lost update anomaly discussed in
\autoref{subsec:internal}.


%
\input{figures/abstract_anomaly}
%























%%
%%
%%
%%
\subsubsection{$\folphi{context}$}
%%
%%
%%
%%
We will first present a set of constraints on variables of our encoding that
must be satisfied by any valid database program. 
These constraints are collectively 
referred to as $\phi_{context}$. 

We first assume,
$\phi_{context}$ enforces $\fol{\omega}$ to respect the
delimitation of transactions. 
More precisely, if a command within a transaction is instantiated, 
all other commands from that transaction must also be instantiated. 
Similarly, the order of commands within transactions must also be respected. 
For example, an instance of {\textcolor{orange}{$\mathsf{payment\_c1}$}} type must
be ordered before a command of type {\textcolor{orange}{$\mathsf{payment\_c2}$}}.

We assume consecutive versions of rows must be associated with different values 
in order to signify any anomalous behaviour at the replaying time. Formally,
\begin{equation}
      \folphi{context}\Rightarrow 
      \forall r,f,n.\;
      \neg(\fol{\rho}_r(f,n)=\fol{\rho}_r(f,n+1))
    \end{equation}
Without this explicit constraint on the values, the solver might trivially
associate all versions to the same constant value which would make 
it more difficult for users to understand the anomaly. 
For example, 
if transaction $\mathsf{twoWrites}$ in \autoref{fig:abstract_anomaly_1}  
is called with parameters $p_1=p_2$,
the dirty value read by $\mathsf{oneRead}$ transaction 
will be equal to the value read in a serializable execution of the two
transactions, which could falsely appear benign to developers.

Now, assuming that $x^{\sql{wh}}$ denotes the
  $\sql{where}$clause of the unique $c\equiv\sql{select}$query that originally
  created $x$, we constrain $\fol{\nu}_x$ such that only rows can be stored in
  $x$ that their witnessed version in $c$ satisfies $c$'s
  $\sql{where}$clause. Formally,
  \begin{equation}
    \folphi{context}\Rightarrow \forall t,r,r_v,n.\;
    \fol{\nu_x}(t,r,r_v,n) \Rightarrow
  \B{x^{\sql{wh}}}{t,c,r,r_v}
  \end{equation}
Notably, we require that all commands, unless they have witnessed a prior
  write operation, must read the initial version of all
  rows. That is, 
      \begin{equation}
       \folphi{context}\Rightarrow 
       (\forall r,f,c_1.\; 
       (\forall c_2.\neg\folwr^{r,f}(c_2,c_1)) \Rightarrow
       \folversionsub{rd}{r,f}(c_1)=0)
     \end{equation}
We enforce causal visibility within replicas:
\begin{equation}
       \folphi{context}\Rightarrow \forall c_1,c_2.\;\ar(c_1,c_2)\wedge (\fol{\tau}(c_1)=\fol{\tau}(c_2))\Rightarrow \vis(c_1,c_2) 
\end{equation}

     
Lastly, we present the remaining components in $\folphi{context}$, constraining 
predicates and variables according to any valid execution of programs:

      \begin{equation}
        \arraycolsep=1.6pt
        \begin{array}{l}
       \folphi{context}\Rightarrow \forall c_1,c_2.\;\vis(c_1,c_2)\Rightarrow\ar(c_1,c_2)  \\
       \folphi{context}\Rightarrow \forall c_1,c_2.\;\folwr(c_1,c_2)\Rightarrow\vis(c_1,c_2)  \\
       \folphi{context}\Rightarrow \forall c_1,c_2.\;\folrw(c_1,c_2)\Rightarrow\neg\vis(c_1,c_2)  \\
       \folphi{context}\Rightarrow \forall c_1,c_2.\;\folww(c_1,c_2)\Rightarrow\ar(c_1,c_2)  
       \\
       \folphi{context}\Rightarrow \forall r,f,c_1,c_2.\; \folwr^{r,f}(c_1,c_2) \Rightarrow
       \folversion{wr}(r,c_1)(f)=\folversion{rd}(r,c_2)(f)
       \\
       \folphi{context}\Rightarrow \forall r,f,c_1,c_2.\; \folrw^{r,f}(c_1,c_2) \Rightarrow
       \folversion{rd}(r,c_1)(f)<\folversion{wr}(r,c_2)(f)
       \\
       \folphi{context}\Rightarrow \forall r,f,c_1,c_2.\; \folww^{r,f}(c_1,c_2) \Rightarrow
       \folversion{wr}(r,c_1)(f)<\folversion{wr}(r,c_2)(f)
       \end {array}
      \label{eqn:exec}
   \end{equation}
























%%
%%
%%
%% 
%%
\subsubsection{$\phi_{DB}$}
%%
%%
%%
%%
We assume a set of user-defined constraints on record instances, 
collectively referred to as $\folphi{db}$.
These constraints might be specified on the \emph{initial version} of the
records, e.g. requiring a table to be initially empty, or on \emph{any version} 
e.g. requiring $\fld{Age}$ field of all records to be always greater than 18. 
Finally, any additional consistency or isolation guarantees (e.g. guarantees
from \autoref{table:consistency_guarantees}) assumed in the
database under test is included in $\folphi{db}$.














%%
%%
%% DEP->
%%
\subsubsection{$\folphi{dep$\rightarrow$}$}
%%
%%
%%
%%

For each pair of commands $\stx{c}$ and $\stx{c'}$
in the given program which could be linked by a dependency relation $\folD$,
$\folphi{dep$\rightarrow$}$ includes a proposition $\eta^{\folD\rightarrow}_{\stx{c,c'}}$. 
This proposition asserts that
\begin{enumerate*}[label=(\alph*)]
\item there exists a concrete row instance that both commands access and
\item both commands are reached by the control flow of their enclosing 
  transactions.
\end{enumerate*}

%
\input{figures/dep_then_rule_example}
%

\autoref{fig:dep_then_rule_example} gives a rule defining a formula that
enforces these conditions when an anti-dependency relation
$\folrw(\stx{c,c'})$ is established between a $\sql{select}$command $\stx{c}$ and
an $\sql{update}$command $\stx{c'}$ which access the same field
$\stx{f}$. The transactions containing the two commands are assumed
to be distinct.
The rule enforces that there is row which satisfies the $\sql{where}$clause of both
commands ($\exists r. \B{\phi}{t,c,r} \wedge~\B{\phi'}{t',c',r}$) and
is perceived alive by them
($\folalive{_{rd}}(r,c)\wedge\folalive{_{rd}}(r,c')$)
and both commands  are reachable 
($\B{\Lambda(c)}{t}\wedge \B{\Lambda(c')}{t'}$).

The full set of rules defining $\eta^{\folD\rightarrow}_{\stx{c,c'}}$ is presented in
\autoref{subsec:fol_rules}. The $\folphi{dep$\rightarrow$}$ clause is simply
defined as their conjunction:
$$\folphi{dep$\rightarrow$} \overset{\Delta}{\equiv}
\bigwedge_{\folD\in\{\folwr,\folrw,\folww\}}\bigwedge_{c,c'\in\opsort}
(\folD(c,c')\Rightarrow\eta^{\folD\rightarrow}_{c,c'})$$





















%%
%% -> DEP
%%
%%
%%
\subsubsection{$\folphi{$\rightarrow$dep}$}
%%
%%
%%
%%
%%
%
\input{figures/delivery}
%
Examining the values of 
$\ar$, $\fol{\tau}$ and $\fol{\rho}$ 
gives us enough information to recover a concrete execution of all the commands
involved in a dependency cycle. 
This suffices for constructing valid test configurations for all the 
examples discussed so far, all of which are consisted of transactions 
that only include commands involved in the dependency cycle. 
Of course, this is not true in general.
In practice, we observed that for the majority of detected anomalies,
transactions include operations which occur 
before the start of the cycle. 
Such operations may cause the database's pre-cycle state to diverge from 
the state assumed by $\folphi{$\mathbb{C}$}$, 
preventing \tool\ from constructing a test configuration that realizes the anomaly.




As an example, consider the $\txn{delivery}$ transaction from TPC-C benchmark,
where records from tables $\mathsf{n\_order}$ and $\mathsf{cust}$ are retrieved 
and updated. 
As presented in \autoref{fig:delivery} (left), 
a lost update anomaly on $\mathsf{cust}$ table may occur if two instances of
$\txn{delivery}$ transaction concurrently select and update the same
$\mathsf{cust}$ record (depicted by red $\folrw$ edges). 
Note that, the primary keys for the retrieved $\mathsf{cust}$ records are determined based 
on the $\mathsf{n\_order}$ records previously selected during steps \ding{172} and \ding{174}.

The above anomaly would be successfully replayed only if \tool\ ensures that 
appropriate $\mathsf{n\_order}$
records exist in the database, such that the select operations at 
steps \ding{176} and \ding{177} are forced to witness the same  $\mathsf{cust}$ record.
Our encoding thus far does not constrain the version of $\mathsf{n\_order}$
record retrieved at step 3, since the $\sql{select}$operation is not on the cycle. 
As a result, \tool\ might falsely assume that the
same (initial) version of an $\mathsf{n\_order}$ record is selected at both steps 
\ding{172} and \ding{174}.
However, if replaying is attempted according to the specified arbitration order,
the $\mathsf{n\_order}$ record retrieved at step \ding{172} will be deleted at
step \ding{173} and will not be witnessed at step \ding{174}.
Consequently, the attempted execution will either terminate or fail to form the desired dependency cycle on
$\mathsf{cust}$.




We remedy this problem via the $\folphi{$\rightarrow$dep}$ clause, 
which forces $\folwr$ edges to exist between
operations that are not part of the dependency cycle. 
When combined with the previous schedule, this clause forces the new
$\folwr$ edge depicted by the green arrow in
\autoref{fig:delivery} (right), 
which in turn 
prevents the operation at \ding{174} to select the same $\mathsf{n\_order}$
record as the one selected
at \ding{173}. 
\tool\ will now make sure two $\mathsf{n\_order}$ records 
exist in the database before the execution begins, both of which refer to the
same $\mathsf{cust}$ record. 





%
$\folphi{$\rightarrow$dep}$ clause 
using the predicate
$\eta^{\rightarrow\folD}_{\stx{c,c'}}$, defines
sufficient conditions under which a dependency relation must exist. 
%
\autoref{fig:then_dep_rule_example} presents the rule that defines the
predicate to force a $\folwr$ dependency when $\stx{c}$ is a 
$\sql{select}$operation and $\stx{c'}$ is an $\sql{update}$such that:
\begin{enumerate*}
\item the update operation is visible to the select,
\item both access the same row, and
\item both $c$ and $c'$ can be executed.
\end{enumerate*}


%
\input{figures/then_dep_rule_example}
%

Using the complete set of rules presented in \autoref{subsec:fol_rules}, 
we can give the full definition of the clause that forces the solver to 
establish dependency edges also between operations outside of a cycle:
$$\folphi{$\rightarrow$dep} \overset{\Delta}{\equiv} 
\bigwedge_{\folD\in\{\folwr,\folrw,\folww\}}\bigwedge_{c_1,c_2\in\opsort}
(\eta^{\rightarrow\folD}_{c_1,c_2} \Rightarrow \folD(c_1,c_2))
$$

















%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Full Dependency Rules}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{subsec:fol_rules}
  Rules defining $\eta^{\folD\rightarrow}$ and $\eta^{\rightarrow\folD}$ are
  presented below. 
  \vspace{4mm}
  
  \centering
%%
 % \hspace{-2.6mm}
  \begin{minipage}[]{.66\textwidth} 
   \begin{mdframed}[backgroundcolor=Main-Theme-Complement]
\vspace{0mm}
  \begin{flushleft}
    \hspace{-2mm}\fcolorbox{black}{Main-Theme-Complement-Dark}{\scriptsize
    \textrm{\sc{\color{black} rw-select-update}}}
  \end{flushleft}
  \vspace{-7mm}
%%

$$
\FOLRULE{
  \stx{c_1 \equiv \sql{select}f\; \sql{as}
  x\;\sql{where} \phi_1 } \\
  \stx{c_2 \equiv \sql{update}\sql{set}
  (f=v)\;\sql{where} \phi_2 } \\
  \stx{
  \folparent(c_1)=t_1 \qquad \folparent(c_2)=t_2 \qquad t_1\not\eq t_2
  \qquad 
  \V{v}{t_2}=(\foldcond_2,\foldval_2)
  }
  \qquad
}
%% ------------------------------------------------------------------------------------------------
  {
  \eta^{\folrw\rightarrow}_{c_1,c_2} =
  \stx{
    \exists r.\;
    \B{\phi_1}{t_1,r,\folversion{rd}(r,c_1)} 
  \wedge \B{\phi_2}{t_2,r,\folversion{rd}(r,c_2)}
  \wedge \folalive{_{rd}}(r,c_1)
  \wedge  
  }
  }
  {
    \stx{
      \folalive{_{rd}}(r,c_2)
  \wedge 
  (\fol{\rho}_{r}(f,\folversionsub{wr}{r,f}(c_2))\!=\!\foldval_2)
    \wedge \foldcond_2
    \wedge \B{\Lambda(c_1)}{t_1}
    \wedge \B{\Lambda(c_2)}{t_2}
    }
  }
$$
\end{mdframed}
\end{minipage}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%%
%%
  \begin{minipage}[]{.66\textwidth} 
    \begin{mdframed}[backgroundcolor=Main-Theme-Complement]
\vspace{0mm}
  \begin{flushleft}
    \hspace{-2mm}\fcolorbox{black}{Main-Theme-Complement-Dark}{\scriptsize
    \textrm{\sc{\color{black} wr-update-select}}}
  \end{flushleft}
  \vspace{-7mm}
%%
$$
\FOLRULE{
  \stx{c_1 \equiv \sql{update}\sql{set}
  (f=v)\;\sql{where} \phi_1 } \\
  \stx{c_2 \equiv \sql{select}(f)\; \sql{as}
  x\;\sql{where} \phi_2} \\
  \stx{
    \folparent(c_1)=t_1 \qquad \folparent(c_2)=t_2 
     \qquad t_1\not\eq t_2
    \qquad
    \V{v}{t_1}=(\foldcond_1,\foldval_1)
  }
}
%% ------------------------------------------------------------------------------------------------
{
  \stx{
    \eta^{\folwr\rightarrow}_{c_1,c_2} =
    \exists r.
    \B{\phi_1}{t_1,r,\folversion{rd}(r,c_1)} 
    \wedge \B{\phi_2}{t_2,r,\folversion{rd}(r,c_2)}
    \wedge \folalive{_{rd}}(r,c_1)
    \wedge 
  }
}
{
  \stx{
    \folalive{_{rd}}(r,c_2)
  \wedge
  ( \fol{\rho}_{r}(f,\folversionsub{wr}{r,f}(c_1))=\foldval_1)
    \wedge \foldcond_1
    \wedge \B{\Lambda(c_1)}{t_1}
    \wedge \B{\Lambda(c_2)}{t_2}
  }
}
$$
\end{mdframed}
\end{minipage}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%%
%
  \begin{minipage}[]{.66\textwidth} 
    \begin{mdframed}[backgroundcolor=Main-Theme-Complement]
\vspace{0mm}
  \begin{flushleft}
    \hspace{-2mm}\fcolorbox{black}{Main-Theme-Complement-Dark}{\scriptsize
    \textrm{\sc{\color{black} {rw-select-insert}}}}
  \end{flushleft}
  \vspace{-7mm}
%%

$$
\FOLRULE{
  \stx{c_1 \equiv \sql{select}f\; \sql{as}
  x\;\sql{where} \phi_1 } \\
  \stx{c_2 \equiv \sql{insert}\sql{values} (\overline{f}=\overline{v}) } \\
  \stx{
    \folparent(c_1)=t_1 \qquad \folparent(c_2)=t_2 \qquad t_1\not\eq t_2 \qquad \V{v(i)}{t_2}=(\foldcond^i_2,\foldval_2^i)
  }
}
%% ------------------------------------------------------------------------------------------------
{
  \stx{
    \eta^{\folrw\rightarrow}_{c_1,c_2} =
    \exists r.
    \B{\phi_1}{t_1,r,\folversion{rd}(r,c_1)} 
    \wedge (\bigwedge\fol{\rho}_{r}(f(i),\folversionsub{wr}{r,f(i)}(c_2))=\foldval^i_2)
    \wedge (\bigwedge \foldcond^i_2)
    \wedge
  }
}
{
  \stx{
    %\neg\folalive{rd}{r}(c_1)
    \folalive{_{wr}}(r,c_2)
    \wedge \B{\Lambda(c_1)}{t_1}
    \wedge \B{\Lambda(c_2)}{t_2}
    %\wedge (\forall n. \neg(\varproj_{\stx{v_{\hat{r}}}}(n,r,t_1)))
  }
}
$$
\end{mdframed}
\end{minipage}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%%
  \begin{minipage}[]{.66\textwidth} 
    \begin{mdframed}[backgroundcolor=Main-Theme-Complement]
\vspace{0mm}
  \begin{flushleft}
    \hspace{-2mm}\fcolorbox{black}{Main-Theme-Complement-Dark}{\scriptsize
    \textrm{\sc{\color{black} {wr-insert-select}}}}
  \end{flushleft}
  \vspace{-7mm}
%%
$$
\FOLRULE{
  \stx{c_1 \equiv \sql{insert}\sql{values} (\overline{f}=\overline{v}) } \\
  \stx{c_2 \equiv \sql{select}f\; \sql{as}
  x\;\sql{where} \phi_2 } \\
  \stx{
  \folparent(c_1)=t_1 \qquad \folparent(c_2)=t_2 \qquad t_1\not\eq t_2 \qquad \V{v(i)}{t_1}=(\foldcond^i_1,\foldval_1^i)
  }
}
%% ------------------------------------------------------------------------------------------------
{
  \stx{
  \eta^{\folwr\rightarrow}_{c_1,c_2} =
  \exists r.
  \B{\phi_2}{t_2,r,\folversion{rd}(r,c_2)} 
    \wedge 
    (\bigwedge \fol{\rho}_{r}(f(i),\folversionsub{wr}{r,f(i)}(c_1))=\foldval^i_1)
  \wedge (\bigwedge \foldcond^i_1)\wedge
}
}
{\stx{
    \folalive{_{rd}}(r,c_1)
    \wedge
    \folalive{_{wr}}(r,c_2)
    \wedge \B{\Lambda(c_1)}{t_1}
    \wedge \B{\Lambda(c_2)}{t_2}
  %\wedge (\exists n. (\varproj_{\stx{v_{\hat{r}}}}(n,r,t_2)))
  }
}
$$
\end{mdframed}
\end{minipage}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%%
  \begin{minipage}[]{.66\textwidth} 
    \begin{mdframed}[backgroundcolor=Main-Theme-Complement]
\vspace{0mm}
  \begin{flushleft}
    \hspace{-2mm}\fcolorbox{black}{Main-Theme-Complement-Dark}{\scriptsize
    \textrm{\sc{\color{black} {rw-select-delete}}}}
  \end{flushleft}
  \vspace{-7mm}
%%
$$
\FOLRULE{
  \stx{c_1 \equiv \sql{select}f\; \sql{as}
  x\;\sql{where} \phi_1 } \\
  \stx{c_2 \equiv \sql{delete}\sql{where} \phi_2 } \\
  \stx{
    \folparent(c_1)=t_1 \qquad \folparent(c_2)=t_2 
  }
}
%% ------------------------------------------------------------------------------------------------
{
  \stx{
    \eta^{\folrw\rightarrow}_{c_1,c_2} =
    \exists r.
    \B{\phi_1}{t_1,r,\folversion{rd}(r,c_1)} 
    \wedge \B{\phi_2}{t_2,r,\folversion{rd}(r,c_2)} 
    %\wedge (\exists n.(\varproj_{\stx{v_{\hat{r}}}}(n,r,t_2)))
  }
}
{
    \wedge \B{\Lambda(c_1)}{t_1}
    \wedge \B{\Lambda(c_2)}{t_2}
    \wedge \folalive{_{rd}}(r,c_1) 
    \wedge \neg\folalive{_{wr}}(r,c_2)
}
$$
\end{mdframed}
\end{minipage}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%%
  \begin{minipage}[]{.66\textwidth} 
    \begin{mdframed}[backgroundcolor=Main-Theme-Complement]
\vspace{0mm}
  \begin{flushleft}
    \hspace{-2mm}\fcolorbox{black}{Main-Theme-Complement-Dark}{\scriptsize
    \textrm{\sc{\color{black} {wr-delete-select}}}}
  \end{flushleft}
  \vspace{-7mm}
%
%%
$$
\FOLRULE{
  \stx{c_1 \equiv \sql{delete}\sql{where} \phi_1}\\
  \stx{c_2 \equiv \sql{select}f\; \sql{as}
  x\;\sql{where} \phi_2} \\
  \stx{
  \folparent(c_1)=t_1 \qquad \folparent(c_2)=t_2  \qquad t_1\not\eq t_2
  }
}
%% ------------------------------------------------------------------------------------------------
{
  \stx{
    \eta^{\folwr\rightarrow}_{c_1,c_2} =
    \exists r.
    \B{\phi_1}{t_1,r,\folversion{rd}(r,c_1)} 
    \wedge \B{\phi_2}{t_2,r,\folversion{rd}(r,c_2)} 
    %\wedge (\forall n. \neg(\varproj_{\stx{v_{\hat{r}}}}(n,r,t_2)))
  }
}
{
    \wedge \B{\Lambda(c_1)}{t_1}
    \wedge \B{\Lambda(c_2)}{t_2}
    \wedge \neg\folalive{_{rd}}(r,c_1) 
    \wedge \neg\folalive{_{wr}}(r,c_2)
}
$$
\end{mdframed}
\end{minipage}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
  \begin{minipage}[]{.76\textwidth} 
    \begin{mdframed}[backgroundcolor=Main-Theme-Complement]
\vspace{0mm}
  \begin{flushleft}
    \hspace{-2mm}\fcolorbox{black}{Main-Theme-Complement-Dark}{\scriptsize
    \textrm{\sc{\color{black} {ww-update-update}}}}
  \end{flushleft}
  \vspace{-7mm}
%
$$
\FOLRULE{
  \stx{c_1 \equiv \sql{update}\sql{set}
  (f=v_1)\;\sql{where} \phi_1 } \\
  \stx{c_2 \equiv \sql{update}\sql{set}
  (f=v_2)\;\sql{where} \phi_2} \\
  \stx{
    \folparent(c_1)=t_1 \qquad \folparent(c_2)=t_2 
  } 
  \quad 
  t_1\not\eq t_2
  \quad 
    \V{v_1}{t_1}=(\foldcond_1,\foldval_1)
  \quad 
    \V{v_2}{t_2}=(\foldcond_2,\foldval_2)
}
%% ------------------------------------------------------------------------------------------------
{
  \stx{
    \eta^{\folww\rightarrow}_{c_1,c_2} =
    \exists r.
    \B{\phi_1}{t_1,r,\folversion{rd}(r,c_1)} 
    \wedge \B{\phi_2}{t_2,r,\folversion{rd}(r,c_2)} 
    \wedge
  (\fol{\rho}_{r}(f,\folversionsub{wr}{r,f}(c_1))=\foldval_1)
  \wedge
  }
}
{
  (\fol{\rho}_{r}(f,\folversionsub{wr}{r,f}(c_2))=\foldval_2)
    \wedge \B{\Lambda(c_1)}{t_1}
    \wedge \B{\Lambda(c_2)}{t_2}
    \wedge \folalive{_{rd}}(r,c_1) 
      \wedge \folalive{_{rd}}(r,c_2)
}
$$
\end{mdframed}
\end{minipage}
%
%
%
%
%
%
%
%
%
%
%
%
%
%%
  
\begin{minipage}[]{.66\textwidth} 
    \begin{mdframed}[backgroundcolor=Main-Theme-Complement]
\vspace{0mm}
  \begin{flushleft}
    \hspace{-2mm}\fcolorbox{black}{Main-Theme-Complement-Dark}{\scriptsize
    \textrm{\sc{\color{black} {insert-select-wr}}}}
  \end{flushleft}
  \vspace{-7mm}
%
%
$$
\FOLRULE{
  \stx{c_1 \equiv \sql{insert}\sql{values} (\overline{f}=\overline{v})} \\
  \stx{c_2 \equiv \sql{select}(f\; \sql{as}
  x\;\sql{where} \phi_2 } \\
  \stx{
  \folparent(c_1)=t_1 \qquad \folparent(c_2)=t_2 \qquad t_1\not\eq t_2 \quad \V{v(i)}{t_1}=(\foldcond^i_1,\foldval_1^i)
}
}
%% ------------------------------------------------------------------------------------------------
{
  \stx{
    \eta^{\rightarrow\folwr}_{c_1,c_2} =
    \exists r.
    \B{\phi_2^w}{t_2,r,\folversion{rd}(r,c_2)} 
    \wedge 
    (\bigwedge \fol{\rho}_{r}(f(i),\folversionsub{wr}{r,f(i)}(c_1))=\foldval^i_1)
  }
}
{
  \stx{
    \wedge (\bigwedge \foldcond^i_1)
    \wedge \B{\Lambda(c_1)}{t_1}
    \wedge \B{\Lambda(c_2)}{t_2}
    \wedge (\not\exists c_3.\; \ar(c_1,c_3)\wedge \folwr^{r,f}(c_3,c_2))
  }
}
$$
\end{mdframed}
\end{minipage}
%
%
%
%
%
%
%
%
%
%
%
%
%
%%
%
%
%
%
%
\vspace{5mm}
\flushleft
Similarly, in \tool\ we define all the following rules:
\\
$\rulelabelinlinec{update-select-wr}$
$\rulelabelinlinec{delete-select-wr}$
$\rulelabelinlinec{update-update-ww}$
$\rulelabelinlinec{insert-insert-ww}$ \\
$\rulelabelinlinec{delete-insert-ww}$
$\rulelabelinlinec{update-update-wr}$
$\rulelabelinlinec{update-delete-wr}$
$\rulelabelinlinec{insert-update-wr}$ \\
$\rulelabelinlinec{insert-delete-wr}$
$\rulelabelinlinec{delete-update-wr}$
$\rulelabelinlinec{delete-delete-wr}$  
$\rulelabelinlinec{wr-update-update}$ \\
$\rulelabelinlinec{rw-update-update}$
$\rulelabelinlinec{wr-update-delete}$
$\rulelabelinlinec{rw-update-delete}$ 
$\rulelabelinlinec{wr-update-insert}$ \\
$\rulelabelinlinec{rw-update-insert}$
$\rulelabelinlinec{wr-delete-insert}$
$\rulelabelinlinec{rw-delete-insert}$






==> sections/full_operational_semantics.tex <==
In this section we will formally define \ir's operational semantics 
and introduce program executions and serializability anomalies.
The syntax of \ir\ is re-introduced in \autoref{fig:syntax_app} for the
readers convenience.

%
\input{figures/ar_syntax_app}
%




%%%%%%%%%%%
\subsection{System Configuration}
%%%%%%%%%%%

Let's assume the set of all database \emph{records} that are present in the replicated table at
any point of time during a finite concurrent execution of a program.
We formally define a record
as a function from field
names to values, denoted by
$\mathfrak{r}:f\rightarrow\intt$.
A record can be unambiguously referred to using its \emph{primary key}.
A primary key $\mathfrak{r}_{k}\in\intt^{|\pk|}$ of row
$\mathfrak{r}$ is composed of the values of $\pk$ columns in $\mathfrak{r}$, 
which are constant across all \emph{versions} of $\mathfrak{r}$.  
%
We define a record version, $\rec_v:f\rightarrow f_v$ as a mapping from
non-$\pk$ fields (i.e. $f\in Fields\backslash\pk$) to natural version numbers, $f_v\in\natt$. 
Version numbers abstract away the set of all modifications a
record witnesses throughout an execution. 
We assume all records are assigned an initial
version (say, $f_v=0$) prior to any operation execution.

%
We define a special non-$\pk$ field $f^\dagger\in Fields\backslash\pk$, whose value (0 or 1)
determines if a particular version of a record is present in the replicated
table (i.e. is alive) or not. As
we will explain in \ir's operational semantics, $f^\dagger$ values can only be
modified by
$\sql{insert}$or $\sql{delete}$operations. 
Records may or may not be alive in their initial version.  




We assume a finite set $\mathcal{R}$ of \emph{replicas}, where each
$\kappa\in\mathcal{R}$
  represents a set of fully connected database nodes that are conjointly disconnected from
  the rest of the database cluster. Effects of operations performed in a replica are
  guaranteed to be witnessed by any later operation in the same replica. 

  We define \emph{events} (denoted by $e$) as follows. 
  A read event, $\rdd{(\rec_k,f,\stx{f_v})}$ is created when an
  operation accesses the field $f$ of a record with key $\rec_k$ and witnesses version
  number $f_v$.
  Similarly, a write event $\wrr{(\rec_k,f,\stx{f_v})}$, is created
  when an operation updates field $f$ of a record to the (higher) version number $f_v$.
  %For technical reasons, we also define insert events, denoted by $\inn{(\rec_k,\rec_v)}$ which can be
  %interpreted as special write events that instantaneously update \emph{all}
  %non-$\pk$ fields of a record.
  Given an event $e$, we denote $e$'s read or written  version on
  field $f$ of the row $\rec_k$, by
  $e^{rd(\rec_k,f)}$ and $e^{wr(\rec_k,f)}$, respectively. Formally,
  $e^{rd(\rec_k,f)}\!=\!f_v$ if and only if $e\!=\!\rdd{(\rec_k,f,f_v)}$, and 
  $e^{wr(\rec_k,f)}\!=\!f_v$ if and only if 
$e\!=\!\wrr{(\rec_k,f,f_v)}$.
%or
%$e\!=\!\inn{(r_k,r_v)}$ where $r_v(f)\!=\!f_v$.



  Similar to \autoref{sec:model}, straightforward control flow handling of 
  \ir\ programs are abstracted away from our
  operational semantics. We instead focus on the details of executing 
  a database operation at a replica. 
  \ir's operational semantics is defined as a small-step relation $(\rightarrow)$
on system configurations, 
defined as $  
    (\Sigma,\vis,\ar,\Theta,I)
$. 
Each element of the configuration is defined below:
\begin{itemize}
  \item $\Sigma:\mathcal{R}\rightarrow\set{e}$
is a map from replicas to disjoint sets of events.
$\Sigma$ is notationally overloaded and is also used to refer to the set of all
events from all replicas, i.e. $\Sigma := \underset{\kappa\in\mathcal{R}}{\bigcup}
\Sigma(\kappa)$.

\item 
$\ar\subseteq\Sigma_{}\times\Sigma_{}$ is an anti-symmetric, irreflexive and transitive \emph{arbitration}  relation 
over the set of events. $\ar$ totally orders all events that are generated
during different execution steps.

\item $\vis\subseteq\Sigma_{}\times\Sigma_{}$ is the \emph{visibility}
  relation between events. $\vis$ is an anti-symmetric and irreflexive relation
  which relates two events if one causally precedes the other. 

\item $\Theta$ captures the set of rows that a client witnesses
and stores following a $\sql{select}\!\!$ query. It is defined
as a mapping from commands to a mapping from set variable
names to tuples of record keys and version numbers, i.e. 
$\Theta: c \rightarrow x  \rightarrow \set{\rec_k\times \rec_v}$.
For example, $\Theta(c_2)(x_1)$ returns the set of all key and version pairs that
a transaction instance witnessed and stored in variable $x_1$, following the
execution of $c_1\equiv(\sql{select}...\;\sql{AS}x_1\;\sql{where}...)$.
$\Theta$ can be thought of as a client-side memory shared between
consecutively executing operations of the same transaction instance.

\item
  $I$ is a step counter which is incremented every time a command is
  executed.
\end{itemize}

Following the literature on weak consistency and isolation 
\cite{todo}, we can specify constraints on $\vis$ and $\ar$ relations, adhering
execution states to
particular operational semantics. \autoref{table:consistency_guarantees_app}
presents a few well-known and massively implemented semantics and their
contracts.
Execution states can be thought of as models for a given
contract.     
For example, an execution state $S$ is linearizable if and only if $S\models \lin$. 

    \input{tables/consistency_guarantees_app}













%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evaluation of Expressions}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Given a transactional program $P$ in \ir\ (i.e. a set of $\stx{txns}$ defined using
the grammar of \autoref{fig:syntax_app}) 
we define an oracle $O^P:=(\omega,\tau,\eta,\rho,\alpha,\beta,\nu)$ as a septuple of partial functions
explained below:
\begin{itemize}
  \item $\omega:\natt \rightarrow c$ is a command instantiation function.
    $\omega(n)$
    returns the command to be processed at step $n$ of an execution.
    $\omega$ satisfies the following properties: 
    \begin{itemize}
    \item  Partially defined on a finite sequence of natural numbers starting from 0.   
    \item  Implicitly spawns a finite number of transactions and respects
    each transaction's internal order when returning its commands. If
    $\omega(c_1)<\omega(c_2)$ and $(c_1)^{txn}=(c_2)^{txn}=t$ then $c_1$ must
    precede $c_2$ in $t$.
    \item Respects each transaction's control flow. Commands encapsulated by
    conditionals must be returned only if those conditions are satisfied.
  \item Respects the loop structures. $\omega$ must unroll and accordingly repeat all contained
    operations in a loop structure based on its iteration count. 
    \end{itemize}
  \item $\tau:  c\rightarrow \kappa$ is a function that maps commands to the
    partition on which they must be executed. 
  \item $\eta:\stx{p} \rightarrow \intt$ is a function that provides concrete
    input arguments to each transaction instance. 
  \item $\rho:(\rec_k\times \rec_v)\rightarrow \rec$ is a function that returns
    concrete values for all versions of records. As we
    will discuss below, our operational semantics does not operate on actual
    values written or read by operations (with the exception of values read from
    or written to $f^\dagger$ field) and instead maintains abstracts versions
    numbers of rows witnessed or updated
    by each operation. 
    %We use $\rho$ to bridge this semantical gap between \ir\ executions
    %and the actual program (e.g. Java) execution.


  \item $\alpha: \mathtt{abs}^{\phi}\rightarrow \intt$ is a function that concretizes
    abstract variables. $\alpha(\mathtt{abs}^{\phi})$ must satisfy the associated
    constraint, $\phi$.

  \item $\beta: \mathtt{iter}\rightarrow \intt$ concretizes iteration variables.
    It keeps track of all loop structures and the number of times each one is
    iterated throughout the execution.

  \item $\nu: (\set{\rec_k\times \rec_v}\times\natt)\rightarrow (\rec_k\times
    \rec_v)$ is a function that totally orders elements of a given set of records
    and their versions. As mentioned in \autoref{sec:model}, we can easily
    extend our query language to support $\sql{order \;by}$constructs which would
    be then manifested as extra constraints on $\nu$.
 %   As explained we will explain below, it facilitates the evaluation of
 %   $\sigma(x,n)$ at runtime.
 
\end{itemize}

An oracle is merely a packaged representation of all sources of non-determinism
occurring in \ir's operational semantics. Given an oracle $(\omega,\tau,\eta,\rho,\alpha,\beta,\nu)$, 
we define deterministic boolean and integer evaluation functions 
  $\B{}{\theta,\delta,\rec_k}:\phi\rightarrow\booll$ 
  and $\I{}{\theta,\delta,\rec_k}:v\rightarrow\intt$  
  in \autoref{fig:i_definition} where the signature of $\theta$ is
  $(x\rightarrow\set{\rec_k\times \rec_v})$ 
  and the signature of $\delta$ is 
  $(\rec_k\rightarrow \rec_v)$. 
  
  As we will explain in the operational semantics rules below, when executing
  a command $c$, $\theta$ can be generated by
  applying $\Theta$ on $c$.  
  Similarly,
  $\delta$ can be generated by applying \emph{view} function, denoted by
  $\Delta^\ar$, on the 
  set of events that are visible to $c$.
  %i.e. the events already present in the
  %replica that $c$ is executing at. 
  View function $\Delta^\ar:\set{e}\rightarrow (\rec_k \rightarrow
  \rec_v)$ is defined to constructs a snapshot of the database
  based on the arbitration order $\ar$ and the set of visible
  events at a replica. $\Delta^\ar(E)$  returns a mapping from each row key to its
  visible version number,
  which is constructed by merging latest update events on
  field of all records in $E$. 
  Formally, given a set of visible events $E$ and for each
  key $\rec_k$ and field $f$, $\;\Delta^{\ar}(E)(\rec_k)(f)=f_v$ if and only if,
$
\mathtt{MAX}^{\ar}_{\rec_k,f}(E)=\{\wrr{(\rec_k,f,f_v)}\}
$
where $ \mathtt{MAX}^{\ar}_{\rec_k,f}(E)=\{e\in E\ALT e=\wrr{(\rec_k,f,\_)} \wedge \neg \ar(e,e')
  \wedge e'\in E
\}$.


\input{figures/full_operational_semantics_I}





  Finally, we define function $\F:\phi\rightarrow\set{\stx{f}}$ in 
  \autoref{fig:f_definition} which recursively extracts all fields that are 
  accessed when evaluating a conditional used in a $\sql{where}$clause.
  $\F$ is used when \ir's operational semantics simulates database-wide scans
  needed for range read and write operations.
%
\input{figures/full_operational_semantics_F} 
%








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Operational Semantics}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The complete operational semantics of \ir\ programs is presented below. 
\\
\begin{center}
\begin{minipage}[b]{.8\textwidth} 
    \begin{mdframed}[backgroundcolor=Main-Theme-Lightest]
\vspace{0mm}
  \begin{flushleft}
    \hspace{-2mm}\fcolorbox{black}{Main-Theme-Lighter}{\scriptsize
    \textrm{\sc{\color{black} e-select}}}
  \end{flushleft}
  \vspace{-8mm}
%
$$
\RULE{
  c=\omega(I) \qquad 
    c \equiv (\sql{select} f\; \sql{as} x\; \sql{where} \phi)
  \\
  \kappa_c=\tau(c) \qquad E=\Sigma(\kappa_c) \qquad
  \delta_{vis}=\Delta^\ar (E) 
    \\
    s =  
    \{(\rec_k,\delta_{vis}(\rec_k)) \ALT 
      \B{\phi}{\Theta(c),\delta_{vis},\rec_k} 
     \wedge 
     \rho(\rec_k,\delta_{vis}(\rec_k))(f^\dagger)=1
 \} 
  \\  

\begin{array}{rll}
  \stx{\varepsilon} & = & 
  \stx{\{\rdd{(\rec_k,f',\delta_{vis}(\rec_k)(f'))}\ALT
      f'\in\F(\phi)\cup\{f^\dagger\}\}}\;\cup
                 \\ &  &
                 \{\rdd{(\rec_k,f,\delta_{vis}(\rec_k)(f))} \ALT
                   \B{\phi}{\Theta(c),\delta_{vis},\rec_k} \wedge
  \rho(\rec_k,\delta_{vis}(\rec_k))(f^\dagger)=1
    \}
\end{array}
  \\
    \Theta' = 
    \Theta [c'\mapsto
    (\Theta(c')[x \mapsto s]) \ALT (c)^{txn}=(c')^{txn}]
  \qquad \qquad \quad 
\\
    \vis' = \vis\cup\{(e_2,e_1)\ALT e_1\in\varepsilon \wedge e_2 \in
    E\}  \qquad 
    \ar' = \ar\cup\{(e_2,e_1)\ALT e_1\in\varepsilon \wedge e_2 \in\Sigma_{}\} 

}
%% ------------------------------------------------------------------------------------------------
{
  \stx{
    \step{(\Sigma,\vis,\ar,\Theta,I)}
    {} %->
    {(\Sigma[\kappa_c\mapsto(\Sigma(\kappa_c)\cup\varepsilon)],\vis',\ar',\Theta',I+1)}
  }
}
$$
\end{mdframed}
\end{minipage}
\end{center}
%
%
%
%
%
%
%
%
%
%
%


\begin{center}
\begin{minipage}[b]{.8\textwidth} 
    \begin{mdframed}[backgroundcolor=Main-Theme-Lightest]
\vspace{0mm}
  \begin{flushleft}
    \hspace{-2mm}\fcolorbox{black}{Main-Theme-Lighter}{\scriptsize
    \textrm{\sc{\color{black} e-update}}}
  \end{flushleft}
  \vspace{-8mm}
%
      
$$
\RULE{
  c=\omega(I)  \qquad 
    c \equiv (\sql{update} \sql{set} f=v\; \sql{where} \phi) 
  \\
  \kappa_c=\tau(c) \qquad E=\Sigma(\kappa_c) \qquad
  \delta_{vis} = \Delta^\ar(E) \qquad \delta_{all} = \Delta^\ar(\Sigma_{}) 
  \\
\begin{array}{rrl}
  \stx{\varepsilon} & = & 
  \stx{\{\rdd{(\rec_k,f',\delta_{vis}(\rec_k)(f'))}\ALT
      f'\in\F(\phi)\cup\{f^\dagger\}\}}\; \cup
  \\ 
  &
  &
  \{\wrr{(\rec_k,f,\delta_{all}(\rec_k)(f)+1)} \ALT
    \B{\phi}{\Theta(c),\delta_{vis},\rec_k}
      \wedge
      \rho(\rec_k,\delta_{vis}(\rec_k))(f^\dagger)=1
    \}
\end{array}
  \\
    \vis' =
    \vis\cup\{(e_2,e_1)\ALT e_1\in\varepsilon
    \wedge e_2 \in E\}
    \qquad 
    \ar' =
    \ar\cup\{(e_2,e_1)\ALT e_1\in\varepsilon
    \wedge e_2 \in \Sigma_{}\} 
}
%% ------------------------------------------------------------------------------------------------
{
  \stx{
    \step{(\Sigma,\vis,\ar,\Theta,I)}
    {}% ->
    {(\Sigma[\kappa_c\mapsto(\Sigma(\kappa_c)\cup\varepsilon)],\vis',\ar',\Theta,I+1)}
  }
}
$$
\end{mdframed}
\end{minipage}
\end{center}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%


\begin{center}
\begin{minipage}[b]{.8\textwidth} 
    \begin{mdframed}[backgroundcolor=Main-Theme-Lightest]
\vspace{0mm}
  \begin{flushleft}
    \hspace{-2mm}\fcolorbox{black}{Main-Theme-Lighter}{\scriptsize
    \textrm{\sc{\color{black} e-insert}}}
  \end{flushleft}
  \vspace{-8mm}
%
$$
\RULE{
  c=\omega(I) \qquad 
    c \equiv (\sql{insert} \sql{values} \overline{f}=\overline{v})
    \\ 
  \kappa_c=\tau(c) \qquad \delta_{all} = \Delta^\ar(\Sigma_{all})
  \qquad   
  \forall_{0\leq i<|\pk|}. \rec_k[i]=\I{\overline{v}[i]}{\Theta(c)} 
    \\
    \forall \rec_v.\; \rec_v(f^\dagger) = \delta_{all}(\rec_k)(f^\dagger)+1 \Rightarrow
    \rho(\rec_k,\rec_v)(f^\dagger)=1
    \\
 \stx{\varepsilon} = 
 \{\wrr{(\rec_k,f, \delta_{all}(\rec_k)(f)+1 )} \;|\; 
 f\in Fields\textbackslash\pk\}
  \\
  \vis' = \vis\cup\{(e_2,e_1)\;|\; e_1\in\varepsilon \wedge e_2 \in \Sigma_{}\} 
   \qquad 
   \ar' = \ar\cup\{(e_2,e_1)\;|\; e_1\in\varepsilon \wedge e_2 \in \Sigma_{}\} 
}
%% ------------------------------------------------------------------------------------------------
{
  \stx{
    \step{(\Sigma,\vis,\ar,\Theta,I)}
    {}% ->
    {(\Sigma[\kappa_c\mapsto(\Sigma(\kappa_c)\cup\varepsilon)],\vis',\ar',\Theta,I+1)}
  }
}
$$

\end{mdframed}
\end{minipage}
\end{center}
%
%
%
%
%
%

\begin{center}
\begin{minipage}[b]{.8\textwidth} 
    \begin{mdframed}[backgroundcolor=Main-Theme-Lightest]
\vspace{0mm}
  \begin{flushleft}
    \hspace{-2mm}\fcolorbox{black}{Main-Theme-Lighter}{\scriptsize
    \textrm{\sc{\color{black} e-delete}}}
  \end{flushleft}
  \vspace{-8mm}
%
$$
\RULE{
  c=\omega(I) \qquad 
    c \equiv (\sql{delete} \sql{where} \phi)
    \\ 
  \kappa_c=\tau(c) \qquad E=\Sigma(\kappa_c) \qquad \delta_{vis} = \Delta^\ar(E)
  \qquad  \delta_{all} = \Delta^\ar(\Sigma_{}) 
  \\
\begin{array}{rrl}
  \stx{\varepsilon} & = & 
  \stx{\{\rdd{(\rec_k,f',\delta_{vis}(\rec_k)(f'))}\ALT
      f'\in\F(\phi)\cup\{f^\dagger\}\}}\; \cup
  \\ 
  &
  &
  \{\wrr{(\rec_k,f^\dagger,f_v)} \ALT
    \B{\phi}{\Theta(c),\delta_{vis},\rec_k}
  \; \wedge \;
      \rho(\rec_k,\delta_{vis}(\rec_k))(f^\dagger)=1 \; \wedge
  \\ 
  & & 
  \; f_v=\delta_{all}(\rec_k)(f^\dagger)+1\;
  \; \wedge \;
  \forall \rec_v. (\rec_v(f^\dagger) = f_v)
   \Rightarrow
  \rho(\rec_k,\rec_v)(f^\dagger)=0    
\}
\end{array}
  \\
    \vis' =
    \vis\cup\{(e_2,e_1)\ALT e_1\in\varepsilon
    \wedge e_2 \in E\} 
    \qquad 
    \ar' =
    \ar\cup\{(e_2,e_1)\ALT e_1\in\varepsilon
    \wedge e_2 \in \Sigma_{}\} 
}
%% ------------------------------------------------------------------------------------------------
{
  \stx{
    \step{(\Sigma,\vis,\ar,\Theta,I)}
    {}% ->
    {(\Sigma[\kappa_c\mapsto(\Sigma(\kappa_c)\cup\varepsilon)],\vis',\ar',\Theta,I+1)}
  }
}
$$

\end{mdframed}
\end{minipage}
\end{center}

\vspace{5mm}
\subsubsection{Remarks on the operational semantics}
The above operational semantics is slightly less permissive than the definition
of bare-bone eventual consistency (EC). 
More precisely, it implements \emph{causal visibility of updates
within a replica (CV)}. 

\begin{wrapfigure}{r}{0.41\textwidth} 
\includegraphics[width=0.4\textwidth]{figures/files/impossible.pdf}
\caption{Execution allowed by EC but not CV}
\label{fig:impossible}
\end{wrapfigure}

Causal visibility enforces that events present in a particular replica are necessarily visible to
the later events occurring in the same replica. 
Note that this model is strictly weaker than causal consistency (CC), as
there is no constraint on the replica an operation can be executed at.
For example, in a pathological case, every
operation from a transaction instance may be executed in its own dedicated
replica without witnessing any of the other events.

We chose this semantics because it precisely models many off-the-shelf key-value data stores. 
Following DynamoDB's system design, these stores implement various anti-entropy
mechanisms which constantly and actively bring stale replicas up to date.   
These mechanisms however, can complicate the task of replaying some executions. 
For example, the execution state presented in \autoref{fig:impossible},
which is allowed under eventual consistency but not CV,
cannot be replayed in Cassandra by mere visibility enforcement through
operation scheduling and static partitioning of replicas.
This execution state can only be reached through dynamic partitioning of
replicas throughout the execution, which we found to be unnecessarily complicated and 
very rare in practice. Utilizing \tool's current replaying solution, 
no matter how operations are associated with partitions and in which order they
are executed, $\mathsf{txn3}$'s update will 
necessarily be visible to both selects from $\mathsf{txn1}$. 
Fortunately, as we will prove in the next subsection, 
our desired anomalous behaviors never impose executions of the above form.
In other words, \ir's operational semantics and \tool's partitioning and scheduling mechanism
are complete in detecting and replaying undesirable serializability anomalies. 










%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\section{Serializability Anomalies}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we formally introduce executions of \ir\ and
potential undesirable behaviors that \tool can automatically detect. 
\subsection{Serial(izable) Executions}
\label{subsec:serializability_anomalies}
Given a program $P$ and an oracle $O^P$, we can construct a
\emph{history} $H=(S_0\rightarrow S_1 \rightarrow ... \rightarrow S_k)$ 
by executing transactions in $P$ according to $O^P$ and against \ir's operational
semantics.
A history is \emph{valid} if $S_0\equiv
(\Sigma_0,\emptyset,\emptyset,\emptyset,0)$ 
and $\forall \kappa\!\in\!\mathcal{R}.\Sigma_0(\kappa)=\{\wrr{(\rec_k,f,0)}\;|\;
\rec_k\in\intt^{|\pk|}\wedge \in Fields\backslash\pk\}$.
In words, all replicas in the initial state of a valid history
must contain a single event for each pair of key and field, which writes
its initial version (i.e. $f_v=0$). 
Optionally, users can further constrain valid histories by specifying a set of
constraints, $\Psi_{\textsc{init}}$,
which must be satisfied by $S_0$.
For example, in TPC-C benchmark, the $ORDER$ table is required to be empty in 
all initial execution states. 
This can be easily enforced by constraining the $\rho$ function to
evaluate initial version of $f^\dagger$ column of all order records to 0, i.e.   $\Psi_{\textsc{init}}:=
\forall \rec_k\in ORDER.\;
\rho(\rec_k,(\lambda f. 0))(f^\dagger)=0$.

We can extend the definition of consistency and isolation properties to a 
set of states $S=\{S_1,S_2,...,S_k\}$ or a history
$H = S_0\rightarrow S_1\rightarrow ... \rightarrow S_k$ if 
all included states satisfy the property. 
In the case of a history, it suffices that only the final state, $S_k$, 
satisfies the property.

Strictly serial histories although ultimately desirable, are extremely costly to
enforce~\cite{pldi15}. 
We instead define a history $H$ to be \emph{serializable} if there exists
a strictly serial history $H'$, that is constructed by reordering
steps of $H$, such that the set of events generated in both
histories are equivalent.

\input{figures/serializability_example_app}

\autoref{fig:serializability_example} presents a serializable execution 
$H\equiv S_0\rightarrow S_1\rightarrow S_2\rightarrow S_3\rightarrow S_4$ on a
single replica
and its equivalent serial execution 
$H'\equiv S'_0\rightarrow S'_1\rightarrow S'_2\rightarrow S'_3\rightarrow S'_4$.
The set of all events in a state $S_i$ is denoted by $\bar{S_i}$. Note that
even though $H$ is not strictly serial (both $\rc$ and $\rr$ are violated), its final set of
events, $\bar{S_4}$, is equivalent to the final set of events in $H'$ which is a
serial execution.

Given a transactional program, our main goal in this paper is to statically define
an oracle whose execution is not serializable, i.e. to
construct a \emph{serializability anomaly}. 
We are specifically interested in finding \emph{independent}
serializability anomalies. A serializability anomaly $H$ is independent, if 
$H\equiv H_1\rightarrow H_2$ where $H_1$ is a valid strictly serial history and $H_2$ 
is a non-serializable history. 
Additionally, we require $H_2$ to be \emph{minimal}.
If the execution of any transaction (i.e. execution of all commands from a
transaction) is not crucial for $H_2$'s non-serializable behavior, then all
such execution steps must
be moved to $H_1$.











%-------------------------------------------------
\subsection{Dependency Cycles}
%-------------------------------------------------


We rely on the ideas of~\citet{AD00} and reduce the problem of
determining serializability of a given execution to the detection of cycles in its
\emph{dependency graph}. 
To this end, we first define three \emph{dependency relations} over the set of events
in an execution state: 
 \begin{itemize}
      \item Read dependency, $\folwr$, relates two events
        if one witnesses a version of a record's field that is
        written by the other. Formally,
        $\folwr(e_1,e_2) \Leftrightarrow \exists \rec_k,f.\; e_1^{wr(\rec_k,f)} =
        e_2^{rd(\rec_k,f)}$.
      \item Write dependency, $\folww$, relates two events if one event overwrites the
        version written by the other on some record's fields. Formally,
        $\folww(e_1,e_2) \Leftrightarrow \exists \rec_k,f.\;
        e_1^{wr(\rec_k,f)}<e_2^{wr(\rec_k,f)}$.
      \item Read anti-dependency, $\folrw$, relates two events if one witnesses
        a version of a record's field, older than the version written by the other. 
        Formally, $\folrw(e_1,e_2) \Leftrightarrow \exists \rec_k,f.\;
        e_1^{rd(\rec_k,f)}<e_2^{wr(\rec_k,f)}$.
    \end{itemize}
We lift the definition of
above dependency relations  (and previously defined $\vis$ and $\ar$
relations) from events to command instances. That is, given an execution state
$S$ and for all relations $\folR\in\{\ar,\vis,\folrw,\folwr,\folww\}$, if 
events $e$ and $e'$ are generate by $c$ and $c'$ in $S$, then 
$\folR(e,e')\Rightarrow\folR(c,c')$.
This lifting is justified, since 
\ir's operational semantics only allows atomic range operations and thus all
events from a command instance are generated at once and hold the same relations
with other events.
We modeled atomic range operations, based on
off-the-shelf eventually consistent data-stores like
Cassandra, which offer users with atomic range operations within a shard while 
strongly encouraging developers to avoid unrestricted multi-shard range queries 
in their application logic and data-models.


We now define a symmetric \emph{same transaction} relation, $\folst$,
relating command instances which are originated from the same transaction
instance. 
We are now ready to define the dependency graph of an execution state $S$, as a
directed  multigraph whose nodes are command instances in $S$ and edges are in
$\{\folrw,\folwr,\folww,\folst\}$.
Following \cite{Nagar:Ser:18} we establish the following necessary conditions
for dependency relations between two commands $c_i$ and $c_j$ from an execution state
$S$:
$$ \Gamma^{c_i,c_j}_{S}\equiv 
      \folww(c_i,c_j) \Rightarrow \ar(c_i,c_j)
      \wedge
      \folwr(c_i,c_j) \Rightarrow  \vis(c_i,c_j)
      \wedge
      \folrw(c_i,c_j) \Rightarrow \neg\vis(c_j,c_i)
      $$

An execution history $H\equiv S_0\rightarrow...\rightarrow S_k$ is non-serializable 
if and only if $S_k$'s dependency graph, $G$, contains a \emph{valid cycle}. 
We define a valid cycle as a 2-regular subgraph of $G$, which 
includes at least two dependency edges (i.e. $\folwr,\folrw,\folww$) and one $\folst$ edge.
Moreover, we do not allow dependency edges between command instances from the same
transaction and w.l.o.g assume they are replaced with $\folst$ edges.
\autoref{fig:cycles_app} presents examples of valid and invalid cycle forms in
dependency graphs. 
\input{figures/cycles_app}
      



We conclude this section by showing that our particular choice of operational 
semantics is permissive enough to manifest all valid dependency cycles 
In other words, given that all other constraints are satisfied, \tool's
replaying mechanism (which preserves causal visibility per partition) is capable 
of replaying all valid dependency cycles (i.e. serializability anomalies).
      
      
\begin{theorem}
      For any  execution state $S$ which manifests a valid dependency cycle $C$,
the necessary constraints imposed by $C$ do not violate causal visibility. 
Formally, 
$$\bigwedge_{c_i,c_j\in C}\Gamma_S^{c_i,c_j} \not\Rightarrow S\models
\neg\cv$$
      
\proof 
      By contradiction. Let's assume such a state and cycle exist. 
      Then it must be the case that:
      $$
      (\bigwedge_{c_i,c_j\in C}\Gamma_S^{c_i,c_j}) 
      \Rightarrow\exists e_1,e_2,e_3\in\bar{S}.\;
      \vis(e_1,e_2)\wedge\vis(e_2,e_3)\wedge\neg\vis(e_1,e_3)
      $$
      Let's assume $e_1$, $e_2$ and $e_3$ are respectively created by
      $c_1$,$c_2$ and $c_3$. 
      Following the atomicity of command execution execution step
      and since $\neg\vis(e_1,e_3)$,
      the following implication trivially holds:
      $$
      (\bigwedge_{c_i,c_j\in C}\;\Gamma_S^{c_i,c_j}) 
      \Rightarrow\exists c_1,c_2,c_3\in\bar{S}.\;
      \vis(c_1,c_2)\wedge\vis(c_2,c_3)\wedge\neg\vis(c_1,c_3)
      $$
      Since $\Gamma^{c_i,c_j}$ only constraints visibility and arbitration
      on $c_i$ and $c_j$, we must have:
      $$\exists c_1,c_2,c_3\in C.\; \Gamma^{c_1,c_2}_S\wedge \Gamma^{c_2,c_3}_S\wedge
      \Gamma^{c_1,c_3}_S \Rightarrow
      \vis(c_1,c_2)\wedge\vis(c_2,c_3)\wedge\neg\vis(c_1,c_3)$$
      By rewriting the left hand side of the implication we arrive at:
      $$\exists c_1,c_2,c_3\in C.\; \folwr(c_1,c_2) \wedge \folwr(c_2,c_3) \wedge \folrw(c_3,c_1) $$
      This is a contradiction since $c_1$,$c_2$ and $c_3$ are on the original
      cycle $C$ but they
      form another cycle of length 3,
      which falsifies 2-regularity of $C$. 
    \end{theorem}



%----------------------------------------   
\subsection{Internal and External Serializability}
\label{subsec:internal}
%----------------------------------------   
During the course of our experiments, we observed that a
subset of serializability anomalies present in database applications,
which we dubbed \emph{external serializability anomalies},
could be considered benign, in that they always leave the final state of the
database indistinguishable from the state after some serializable execution of
the same instances. 
The key observation here is that some of the read events in a non-serializable
execution, do not affect the transactions' control flow or any of the later
write events. 
As a result, those events (denoted by $\rddp{}$) could be excluded from the
correctness analyses, in order to only detect the
more harmful \emph{internal serializability anomalies}. All internal serializability
anomalies leave the database state permanently diverged from a serializable 
execution state and must be carefully studied and addressed by the developers. 

%%
\input{figures/abstract_anomaly2_app}
%%

\autoref{fig:abstract_anomaly2} presents two executions $H$ (left) and $H'$
(right). $H$ is consisted of two instances of $\mathsf{upd}$
transaction, within which the variable $\mathsf{x}$ is read and
is then updated to a fresh value. 
Similarly, $H'$ includes two instances of $\mathsf{inc}$ transaction
where the value of $\mathsf{x}$ is read and then is \emph{incremented}
by 10.
Both of these executions are non-serializable as they manifest the
lost update anomaly. However, only $H'$ includes an internal
serializability anomaly, where the database is left in a state that
is inconsistent with any serializable executions.

Various models of application tolerance for temporarily inconsistent
views of the global database state (in exchange for higher availability 
and throughput) have been formulated and introduced in the literature of weak
consistency and memory models from 2010s.
For instance, the popular CRDT-based programming model~\cite{crdt} has been 
solely developed around the idea of explicitly allowing stale views of the 
database throughout executions, with the additional guarantee of eventual
convergence, a.k.a \emph{strong eventual consistency}.  
Similarly, in the context of weak memory models, 
certain conflicting data access patterns have been deemed safe by
various atomicity violation detection techniques (e.g. \cite{Lucia:ColorSafe:2010}) 
due to lack of data flow between the read and write operations involved in the
conflict. 


To the best of our knowledge, we are the first 
to systematically formulate internal serializability, IS, as a fine-grained
semantic property of abstract executions and incorporate in \tool for detection
of safety violations in modern database applications.































==> sections/proofs.tex <==
\begin{lemma}
If the FOL formula is not SAT, then there is no anomalous abstract execution.
\end{lemma}
%
%
\begin{theorem}
(Soundness) for every model of the FOL formula there exists an anomalous execution.
\end{theorem}
\begin{theorem}
(Completeness) Our search algorithm finds ALL anomalous executions within the given bounds
\end{theorem}


==> tables/consistency_guarantees_app.tex <==
% settings
%\setlength{\arrayrulewidth}{0.5pt}
%\setlength{\tabcolsep}{4pt}

\def\arraystretch{1}
% table
\begin{table}[b!]
\centering
\begin{footnotesize}
{\rowcolors{1}{Main-Theme-Light}{Main-Theme-Lighter}
  \begin{tabular}{|l | l |} 
 \hline
 \rowcolor{Main-Theme-Dark}
    Guarantee Name & 
    \multicolumn{1}{c|}{Specification} 
   \\
 \hline
     Causal Visibility & $\cv \equiv \vis(e,e')\wedge\vis(e',e'')
    \Rightarrow \vis(e,e'')$ \\
     Causal Consistency & $\cc \equiv \cv\wedge (\st(e,e') \Rightarrow
     \vis(e,e')\vee \vis(e',e))$ \\
     Read Committed  & $\rc  \equiv \st(e,e') \wedge \vis(e,e'') \Rightarrow
    \vis(e',e'') $\\
     Repeatable Read &  $\rr  \equiv \st(e,e') \wedge \vis(e'',e) \Rightarrow
    \vis(e'',e') $ \\
     Linearizable & $ \lin  \equiv \ar \subseteq \vis $ \\
    Strictly Serial & $ \ser \equiv \rc \wedge \rr \wedge \lin$ \\
    [0.3ex] 
 \hline
\end{tabular}
}
\end{footnotesize}
\vspace{2mm}
  \caption{Consistency and isolation guarantees}
\label{table:consistency_guarantees_app}
\end{table}


